Age of Information and Energy Consumption in IoT: an Experimental Evaluation

The Age of Information (AoI) is an end-to-end metric frequently used to understand how "fresh" the information about a remote system is. In this paper, we present an experimental study of the relationship between AoI and the energy spent by the device that produces information, e.g. an IoT device or a monitoring sensor. Such a relationship has been almost neglected so far, but it is particularly important whenever the sensing side is battery-operated. The study is carried out in a scenario where access is achieved via the cellular network and information is transferred using MQTT, a popular messaging protocol in the IoT domain. Numerous parameters of operation are considered, and the most efficient solutions in all configurations are provided.

==> thesis-sections/aoi.tex <==
\section[Energy Consumption and Age Of Information: a combined study]{Energy Consumption and AoI:\\a combined study}

The second experiment campaign regards the combined study of the two metrics of interest, namely the energy and the \acrshort{aoi}. As highlighted in \ref{chap:related-works} an experimental measurement of both metrics has not yet been extensively studied, so these experiments aim to fill this gap by analyzing possible differences of \acrshort{mqtt} on top of \acrshort{tcp}/\acrshort{tls} and \acrshort{quic} transport protocol. As for the first experiment campaign the \acrshort{tls} version is the latest available, i.e. 1.3.

The \acrshort{aoi}, already introduced in \ref{chap:introduction}, is an appropriate metric to evaluate the freshness of information owned by a collection point, which may be a service placed in the cloud that applies time-sensitive logic to the data collected by \acrshort{iot} nodes. A common scenario is an \acrshort{iot}-based monitoring and control system that takes actions based on the data gathered by the sensors deployed in the sensing environment and produces commands in response to the information extracted by the data. In this scenario, having fresh data is critical to making the right decisions and issuing the most appropriate commands to system actuators responding promptly to changes in the environment. When some analysis is performed on \acrshort{iot} systems the energy constraint must always taken into account because it poses a limit on the optimisation of the other metrics. Having fresh information can be critical for many applications, but if obtaining the minimum \acrshort{aoi} the nodes deplete their battery very quickly the system won't be able to receive any information after a short period of activity, requiring a human intervention to replace exhaust batteries. This approach is not convenient because the human intervention limits the benefits of an \acrshort{iot} system where at least the monitoring is automated, moreover, there may be applications for which battery replacement is not possible or is very expensive. For these reasons, the \acrshort{aoi} is directly evaluated jointly with the energy consumption contrary to the latter that has been previously studied independently.

The experiment scenario is different from the one of the energy experiment campaign because now it's interesting to observe the \acrshort{aoi} evolving in time and only after extracting statistics from the time evolution to summarise the data. Moreover analysing the metric over a time window allows a faithful reproduction of the scenario referenced in the experiment and repeating the same operation in the experiment ensures a more robust statistical significance of the collected data. These considerations lead to a new working flow for the device under test, i.e. the \acrshort{rpi} that produces and sends \acrshort{mqtt} messages:
\begin{enumerate}
	\item Client sends connect message to the broker
	\item Client waits for connection acknowledgement from the broker
	\item Client periodically publishes a message to the broker, adopting a pipelining mechanism
	\item Client sends a disconnect message to the broker once all the configured messages and relative acknowledgements have been correctly received
\end{enumerate}

The pipelining mechanism, a name borrowed by the same technique implemented in the \acrshort{http}/1.1 protocol \cite{http11}, is depicted in \ref{fig:pipelining} and its adoption stems from the observation that waiting for an acknowledgement before sending a new message limits the transmission rate to the inverse of the \acrshort{rtt} of the network. The limitation stems from the fact that the acknowledgement is sent in response to the publisher's message, so in the best case, it's necessary to pay twice the one-way delay of the network to receive the broker's response correctly. If the new message can be sent only after the acknowledgement reception then the minimum period between two messages will be equal to \acrshort{rtt} and thus the maximum rate will be the inverse of that period.

\begin{figure}
    \centering
    \begin{subfigure}{0.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/aoi/no-pipelining.pdf}
        \caption{No pipelining} 
        \label{fig:pipelining-off}
    \end{subfigure}%
    \begin{subfigure}{0.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/aoi/pipelining.pdf}
        \caption{Pipelining} 
        \label{fig:pipelining-on}
    \end{subfigure}%
    \caption{Pipelining mechanism for three \acrshort{mqtt} publish messages}
    \label{fig:pipelining}
\end{figure}

The pipelining mechanism is implemented in the second version of the client tools developed for this thesis, the custom stream-client presented in \ref{sec:client-tool}, which as already described is designed to publish multiple messages with a given rate before exiting. A brief guide to using the stream-client tool is provided in \ref{sec:command-line-tool} of the appendix.

Finally, a last remark on the importance assumed by the synchronization between publisher and subscriber, i.e. the \acrshort{rpi} and the laptop. The computation of \acrshort{aoi} is possible only if both the instant of message generation and reception are recorded, the first on the \acrshort{rpi}, the second on the laptop. The difference between the two timestamps is the \acrshort{aoi} at the message arrival, but if the clocks of the two devices are not synchronized the time offset would be considered in the difference, producing an inaccurate result. For this reason, synchronization is fundamental for these experiments. The synchronization problem is represented in \ref{fig:sync-problem} to better understand the consequences of a clock offset.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/clock-offset.pdf}
    \caption{Synchronization problem for the \acrshort{aoi}}
    \label{fig:sync-problem}
\end{figure}

\subsection{Experiments}
In \ref{tab:aoi_parameter_space} a summary of the explored parameter space is reported. The configuration of each experiment consists of the same parameters as the first set of experiments, except for the cellular technology. In addition to these parameters others are added:
\begin{itemize}
    \item \textbf{Time window}, it is the nominal duration of the experiment after which the client can exit.
    \item \textbf{Queue policy}, it is the configuration of the queue between the task that generates the messages and the one that sends them over the network, according to the architecture described in \ref{sec:client-tool}.
    \item \textbf{Generation rate}, it is the nominal rate at which the \acrshort{rpi} generates and thus tries to publish the messages toward the broker.
    \item \textbf{CPU cores}, as pointed out in \ref{chap:setup} the \acrshort{rpi} is equipped with a 4-core CPU even if the majority of experiments have been carried out with only one core enabled.
\end{itemize}

Note that the actual generation and transmission rates may be different from the nominal ones due to the lack of computing or network resources. The number of messages to be sent during the experiment is fixed, computed as the nominal rate multiplied by the time window, so in case a lower rate is reached the duration of an experiment may exceed the planned one.

The rate's values were chosen to take into account the shape of \acrshort{aoi} as the transmit rate varies, according to what is described in \ref{chap:related-works}. Initially, the metric should improve rapidly as the rate increases and then, once the minimum value is reached, it should slowly rise again to a saturation point. The values are therefore chosen following a linear scale with a step of 1000, but to better observe the initial descent the values 10 and 100 are added. The values choice was supported by some preliminary experiments carried out to roughly observer the trend of \acrshort{aoi}. From these tests also came out that 60 seconds for the time window were more than sufficient to observe a significant time evolution of the metric. Finally, the payload size considered is only 128 bytes because is a suitable size to accommodate a wide range of sensor measurements in the \acrshort{iot} domain. Note that only a subset of the cartesian product of the parameters space has been tested.

Regarding the queue policies the ones explored are \acrfull{fifo}, for three different sizes, and head-drop. The \acrshort{fifo} policy is the standard management of a queue, the messages are extracted from it in the same order they enter and thus are sent in the same order as they were generated. Moreover, a quite important observation is that this policy doesn't expect any of the generated messages to be lost. They are queued as long as there is space available, but when the queue is full the producer will have to wait before adding another message. The space in the queue may have a significant effect on the results, so three different sizes are selected. The sizes should represent three levels of queue length, i.e. large, medium and no queue. The queue with only one position doesn't allow the insertion of a message before the previous one has already been sent, for this reason, it can be considered as having no queue in the system. The literature, as already analysed in \ref{chap:related-works}, shows that the \acrshort{aoi} can be optimized with a \acrfull{lifo} policy. This scenario deserves to be explored, however is important to take into consideration that usually the \acrshort{aoi} metric is relevant for control systems, for which the reception of an old message after a new one could be useless. This consideration led to the head-drop queue policy, i.e. the queue is transformed into a simple buffer that can be overwritten by a new message if the old one has not yet been extracted. Apart from the effect on \acrshort{aoi}, the head-drop queue has another impact on the experiments as the policy allows for losses of messages contrary to the \acrshort{fifo} one. A consideration of the system's requirements and the queuing policy is necessary since the two strategies meet different requirements: the head-drop policy is suitable for a system requiring only fresh data, whereas the \acrshort{fifo} policy is suitable for a system in which the data series is also valuable, e.g. if the logic works with a group of consecutive data rather than a single sample, and therefore a hole in the series may not be accepted. 

Finally, it is worth highlighting that the queues referenced operate at the application level, even if other queues, which are typically handled via the classic \acrshort{fifo} policy, are present at a lower level in the system. These queues have been analysed by other works but for this thesis, the idea is to work only at the application level without getting involved in kernel optimization. This choice is justified by the fact that in a real application, there are many requirements and the development time is often one of the most stringent to meet. Working at the kernel level thus may be quite often not feasible, so the analysis is restricted to the application level while being aware that there would potentially be many other aspects to deal with.

\begin{table}
	\centering
	\caption{\acrshort{aoi} experiment parameter space}
	\begin{tabular}{lcl}
		\toprule\toprule
		\multicolumn{1}{c}{\textbf{Parameter}} & \multicolumn{1}{c}{\textbf{Unit of Measure}} & \multicolumn{1}{c}{\textbf{Value}} \\
		\midrule
		Transport protocol & - & \acrshort{tls} (v1.3), \acrshort{quic} \\
		\midrule[0pt]
        Payload size & [B] & 128, 256, 512, 1024, 2048 \\
		\midrule[0pt]
		Delay & [ms] & 0, 20, 40, 60, 80 \\
        \midrule[0pt]
		Bandwidth & [Mbit/s] & 100\%\footnotemark \\
        \midrule[0pt]
        Access network& - & 4G \\
        \midrule[0pt]
        Time window & [s] & 60\\
        \midrule[0pt]
        \multirow{2}{*}{Queue policy} & \multirow{2}{*}{-} & FIFO 1024, FIFO 16,\\  & & FIFO 1, HEAD-DROP\\
        \midrule[0pt]
        \multirow{2}{*}{Generation rate} & \multirow{2}{*}{[msg/s]} & 1, 10, 100, 1000, 2000, 3000,\\ & & 4000, 5000, 6000, 7000, 8000 \\
        \midrule[0pt]
        CPU cores & - & 1, 2 \\
		\bottomrule
	\end{tabular}
	\label{tab:aoi_parameter_space}
\end{table}
\footnotetext{No bandwidth restriction}

\subsection{Statistics on AoI}
The recording of generation and reception instants of the message published during the time window gives all the information needed to compute the \acrshort{aoi} not only in correspondence with the message arrival but in any instant along the entire duration of the experiment, obtaining an exact form for the sawtooth shape function that characterises the metric. Dealing with an analytic expression of the function, rather than a discrete group of points, e.g. by sampling the time evolution of \acrshort{aoi}, allows for precise calculations of the statistical quantities, needed to aggregate the collected data for the analysis. The drawback is that those calculations might be not straightforward to implement. The statistical quantities taken into consideration are mean and median values.

\subsubsection{Time evolution}
The formula applied to compute the exact value of the \acrshort{aoi} in each instant is reported in \ref{eq:aoi-formula}.
\begin{equation}
    \Delta(t)=t - U(t),\quad
    \begin{cases}
    \Delta(t)\rightarrow\textit{\acrshort{aoi} at instant t}\\
    U(t)\rightarrow\textit{Generation time of the newest data received}
    \end{cases}
    \label{eq:aoi-formula}
\end{equation}

The shape of \acrshort{aoi} function is quite distinctive because from the definition of the metric some properties are guaranteed and can be leveraged during the computations. More precisely, it assumes an irregular sawtooth shape, rising linearly while waiting for new messages and then upon the arrival of a message it suddenly falls to a lower value, but despite this, the following properties hold:

\begin{itemize}
    \item The function is always positive, with a lower bound given by the one-way delay of the network.
    \item Each linear section has a $45^\circ$ inclination, i.e. slope 1, so the distance covered on the x-axis is the same as the one on the y-axis for each segment.
    \item The function is integrable.
\end{itemize}

The first property is trivial, the \acrshort{aoi} can't assume negative values from construction since it represents the freshness of information and the minimum time required for a message to reach the receiver, i.e. the delay of the network, represents a lower limit for the function. The second one derives directly from the definition of the \acrshort{aoi} because if no messages arrive the available information after a certain amount of time will be aged of the same quantity. The last property is obtained by observing that the function falls at least in the class of integrable functions having finite numbers of discontinuity points since the only points, close to the arrivals of messages that cause a jump in the function.

The presented formula can easily implemented by software via a simple loop over the timestamps collected during the experiments. For each message, the start-point of the segment is computed as the difference between generation and reception timestamps, and jointly with the latter defines a tuple that will be added to a vector. The vector contains the exact points of \acrshort{aoi} at the message arrivals, but applying the above formula is sufficient to obtain the exact value at each instant. 
Leveraging the function's special properties, the time evolution can be graphed using any standard tool by simply building an array containing the start and end point of each linear section that composes the function.

\subsubsection{Mean Value}
The mean value is the simplest form of data aggregation. However, dealing with a function requires a different approach than the simple arithmetic mean applicable for a discrete set of points, as in the case of the first set of experiments. The first solution is the sampling of the \acrshort{aoi} function, which results in a series of discrete points on which the arithmetic mean is applicable. This simple solution leads to an approximation of the mean value sought, which might be sufficient in principle, but having a simple analytical expression of the function allows a better approach that comes from mathematical analysis theory. The mean of a function can be computed leveraging the definition of integral mean, reported in \ref{eq:integral-mean}, which states that the integral mean of a function over an interval is the ratio of the definite integral of the function over the interval to the length of the interval.

\begin{equation}
    \begin{aligned}
        &f : [a, b] \rightarrow\mathbb{R}\textit{ bounded and integrable in } [a,b] \\
        &M(f,[a,b])=\frac{1}{b-a} \int_{a}^{b} f(x) \, dx
    \end{aligned}
\label{eq:integral-mean}
\end{equation}

The definition requires the integrability of the function on the considered interval, but as already noted, this property is always satisfied by construction. The length of the interval is given by the time elapsed between the first and last message received by the subscriber, i.e. the difference between the x-coordinates of the points at the extremes of the \acrshort{aoi} function. As far as the definite integral is concerned, its calculation exploits the properties of the function's shape. Firstly, the function is always positive, so the integral represents the area under the curve. Therefore, the area can be calculated as the sum of the areas under each segment, which results in calculating the area of multiple right-angled trapezoids. Referring to the \ref{fig:integral-mean}, the area of each trapezoid can be calculated by adopting one of the two following approaches:

\begin{itemize}
    \item Sum of the areas of a rectangle and a triangle as in \ref{fig:mean-1}. The length of the rectangle is the inter-arrival time between two messages, computed as the difference of the reception timestamps and the height is the starting \acrshort{aoi} value, i.e. the one computed at the arrival of the first message among the two into consideration. Regarding the triangle, the base is again the inter-arrival time between messages, while the height is the vertical difference between the starting \acrshort{aoi} and the maximum value reached before the jump, but recalling the properties of the function the horizontal distance is the same of the vertical one, thus the value is the same of the inter-arrival one.
    \item Area of the rectangle having a height equal to the y-coordinate of the midpoint of the segment as in \ref{fig:mean-2}. The rectangle may appear to leave out a small triangle at the top right and include an extra one at the bottom left, but after a simple geometric analysis, it can be shown that the two triangles are equivalent, so the calculation returns the correct value of the area. 
\end{itemize}

\begin{figure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/aoi/mean_aoi_1.pdf}
        \caption{Integral mean method-1} 
        \label{fig:mean-1}
    \end{subfigure}%
    \begin{subfigure}{0.45\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/aoi/mean_aoi_2.pdf}
        \caption{Integral mean method-2} 
        \label{fig:mean-2}
    \end{subfigure}%
    \caption{Integral mean for \acrshort{aoi} function}
    \label{fig:integral-mean}
\end{figure}

The implementation of the two approaches is very similar, both require a simple loop over the generation and reception timestamps.

In \ref{tab:integral-sampling-mean}, some examples of the difference between integral mean and arithmetic mean over a sampled, 1000 samples per second, function are reported. 
\begin{table}
  \centering
  \caption{Difference between integral and arithmetic mean for \acrshort{quic}, FIFO-16 configurations}
  \label{tab:integral-sampling-mean}
  \begin{tabular}{lrrr}
    \toprule\toprule
    \textbf{Configuration} & \textbf{Integral Mean [ms]} & \textbf{Arithmetic Mean [ms]} & \textbf{Difference [ms]} \\
    \toprule
    Rate 1 & 551.12 & 550.61 & 0.51 \\
    \midrule[0pt]
    Rate 10 & 95.60 & 95.10 & 0.50\\
    \midrule[0pt]
    Rate 100 & 72.03 & 71.55 & 0.48\\
    \midrule[0pt]
    Rate 1000 & 50.08 & 49.63 & 0.45\\
    \bottomrule
  \end{tabular}
\end{table}

\subsubsection{Median Value}
The median value is the second form of data aggregation defined for the \acrshort{aoi} function, introduced to obtain a value more robust to noise than the mean. The problem is to find an extension of the median applicable to a function and not to a discrete set of points, obtaining the same type of relationship that exists between the arithmetic mean and integral mean. The median is defined as the value separating the higher half from the lower half of the points in the set. The concept of half the points of the set can be extended to half the length of the interval over which the \acrshort{aoi} function is defined. Based on this new definition, the median value can be assumed as the level of \acrshort{aoi} for which the sum of the lengths of the intervals on the x-axis that have associated \acrshort{aoi} less than (greater than) the median is exactly half of the total length of the interval over which the function is defined. The visualization of this definition is reported in \ref{fig:aoi-median-definition}. 

\begin{figure}
    \centering
    \includegraphics[width=0.85\columnwidth]{images/aoi/median_definition.pdf}
    \caption{Median definition for \acrshort{aoi} function}
    \label{fig:aoi-median-definition}
\end{figure}

Once established how to interpret the median for the \acrshort{aoi} function, the problem is to find a method to compute such value. Before analysing the possible methods, is worth highlighting that despite the difficulty of computing the median value, the check on it is quite easy. Knowing all the points of the \acrshort{aoi} function, given a value on the y-axis, i.e. the median, is sufficient to check the length of each segment below the given value and normalize it to the total length of the function. The computation will result exactly in one-half if the given value is the sought median.

\subsubsubsection{Analytic method}
The mathematical formulation of the median problem, following the definition above, is quite simple knowing the shape of the function. The problem is to find for each linear section of the \acrshort{aoi} function the fraction of the segment below the unknown median value, expressed as a parameter in the interval zero-one. A zero parameter means that the segment is completely above the median value, i.e., that for that period the \acrshort{aoi} was always greater than the median \acrshort{aoi}, while the opposite is true for a parameter one. The analytic expressions of the segments are easy to find because every point of the \acrshort{aoi} function is known, so they are simply expressed as a segment between two points. The only missing unknown is the median value sought, but it can be imposed by requiring that the sum of all partial segments result in exactly half the interval over which the \acrshort{aoi} function is defined.
By enclosing all the previous equations, the median will be expressed by a linear system that has as many equations as there are unknowns. Referring to the \ref{fig:aoi-median-definition} an example of the system is reported in \ref{eq:median-system}. The median is represented by the unknown $m$, while the parameters which determine the portion of segments below the median are expressed by the Greek letters.   

\begin{equation}
    \label{eq:median-system}
    \begin{cases}
        (b_x - a_x)\widehat{\alpha} + (d_x - c_x)\widehat{\beta} + (f_x - e_x)\widehat{\gamma} = T/2 \\
        a_y + (b_y - a_y)\widehat{\alpha} = m \\
        c_y + (d_y - c_y)\widehat{\beta} = m \\
        e_y + (f_y - e_y)\widehat{\gamma} = m 
    \end{cases}
\end{equation}

In general, the solution might be computed by inverting the matrix of coefficients, but it doesn't have a negligible cost. However, again from properties of the \acrshort{aoi} function, the system can easily be solved by leveraging the unitary slope. The final expression for the median and the parameters is reported in \ref{eq:median-system-solved}. 

\begin{equation}
\label{eq:median-system-solved}
\begin{cases}
    (b_x - a_x)\frac{m - a_y}{b_y - a_y} + (d_x - c_x)\frac{m - c_y}{d_y - c_y} + (f_x - e_x)\frac{m - e_y}{f_y - e_y} = T/2 \\
    \widehat{\alpha} = \frac{m - a_y}{b_y - a_y} \\
    \widehat{\beta} = \frac{m - c_y}{d_y - c_y} \\
    \widehat{\gamma} = \frac{m - e_y}{f_y - e_y} 
\end{cases}
\end{equation}

By observing that the difference between the x and y components is the same, from the unitary slope, the first equation of the above system can be simplified, removing all the fractional parts, as reported in \ref{eq:median-system-optimised}. The trivial form of the system obtained requires a few simple operations to retrieve the wanted values. 

\begin{equation}
\label{eq:median-system-optimised}
\begin{cases}
    m - a_y + m - c_y + m - e_y = T/2 \\
    \widehat{\alpha} = \frac{m - a_y}{b_y - a_y} \\
    \widehat{\beta} = \frac{m - c_y}{d_y - c_y} \\
    \widehat{\gamma} = \frac{m - e_y}{f_y - e_y} 
\end{cases}
\end{equation}

The system, for which the only possible solution is easily obtained, so far lacks an important piece, which should be checked a-posteriori, namely, the conditions limiting the parameters in the zero-one interval. If these conditions aren't met the computed value for the median won't be correct, so they should be imposed directly during the resolution of the system. Imposing such conditions, as reported in \ref{eq:median-system-constrained}, leads to a system that is not more linear and its resolution cannot be obtained via a matrix inversion or adopting the optimized computation above described. 

\begin{equation}
    \label{eq:median-system-constrained}
    \begin{cases}
        (b_x - a_x)\widehat{\alpha} + (d_x - c_x)\widehat{\beta} + (f_x - e_x)\widehat{\gamma} = T/2 \\
        a_y + (b_y - a_y)\widehat{\alpha} = m \\
        c_y + (d_y - c_y)\widehat{\beta} = m \\
        e_y + (f_y - e_y)\widehat{\gamma} = m \\
        \widehat{\alpha} \geq 0 \\ 
        \widehat{\beta} \geq 0 \\
        \widehat{\gamma} \geq 0 \\
        \widehat{\alpha} \leq 1 \\
        \widehat{\beta} \leq 1 \\
        \widehat{\gamma} \geq 1 
    \end{cases}
\end{equation}

\subsubsubsection{Bisection method}
Solving the system may be quite difficult and involve advanced techniques, not taken into consideration for this thesis.
A possible different approach might be based on an approximation of the median value via an iterative procedure, such as a variation of the bisection method. The method consists of choosing a starting tentative median chosen in the maximum-minimum \acrshort{aoi} interval and checking which fraction of the function falls below the tentative value. If the fraction is above half, then the considered interval shrinks between the minimum of the previous interval (the minimum \acrshort{aoi} after the first cycle) and the current tentative median, otherwise between the latter and the maximum of the previous interval (the maximum \acrshort{aoi} after the first cycle). The procedure stops once the check results in a fraction below an established threshold. The approximation will be as accurate as the threshold is near to one-half, considering a normalized \acrshort{aoi} function interval, but it will require also a higher number of cycles.

\subsubsubsection{Projection method}
The bisection method is easy to implement, but the value obtained is just an approximation of the median value. It is a general procedure that can be applied to any function, but leveraging the properties of the \acrshort{aoi} function makes it possible to obtain the exact value for the median without involving complex computations. The exploited property is once again the unitary slope that allows interchangeable work on both the x-axis and y-axis. The method is based on the projection of each segment on a vertical axis, referred to as the projection axis. The projections on this axis will probably generate some overlapping regions, i.e. for a certain interval on the axis more than one projection (or at least a fraction of it) will fall on it. For each region, identified by the intersections of the projections, a weight is assigned, computed as the number of different projections that fall on it. Once the construction of the projection axis is completed the next step is to compute a weighted sum as the length of each region times the associated weight, which will be referred to as total extension. The last step is to iterate over the regions, from bottom to up, computing their extension, i.e. length by weight and summing it up until half of the total extension is reached. The last sum will probably exceed the half of total extension, so only a fraction of the length of the last region, multiplied by the associated weight, is to be considered. The point on which the iteration stops, i.e. the quote on the y-axis, is the median value. The construction of the projection axis is reported in \ref{fig:projection-algorithm} and an implementation of the algorithm is shown in Algorithm \ref{alg:median}. Note that the correctness of the algorithm comes from the fact that the vertical shift can be considered instead of the horizontal one since the slope is the same for all segments. This property is exploited to count how many times a projection falls in a region, but this would not be possible when working only on the x-axis. Recalling the standard procedure to compute the median for a discrete set of points, the required steps are to order the points and then select the one in the middle. This procedure perfectly matches the one adopted in the second part of the presented algorithm, with the exception that the set is composed of intervals (regions), and not discrete points and the counting takes into consideration the extension of the region and not the number of regions in the set.

\begin{figure}
    \centering
    \includegraphics[width=0.85\columnwidth]{images/aoi/median_projection_axis.pdf}
    \caption{Projection algorithm}
    \label{fig:projection-algorithm}
\end{figure}

\begin{algorithm}
\caption{Projection median}
\label{alg:median}
\begin{algorithmic}
    \Function{compute\_projection\_median}{$\textit{timestamps}$} \Comment{Returns a float}
        \State $\textit{projections} \gets \text{empty list}$
        \State $\textit{extension} \gets 0$

        \For{$i \gets 1$ to $\text{len}(\textit{timestamps}) - 1$}
            \State $\textit{start\_aoi} \gets \textit{timestamps}[i - 1]["rx"] - \textit{timestamps}[i - 1]["gen"]$
            \State $\textit{end\_aoi} \gets \textit{timestamps}[i]["rx"] - \textit{timestamps}[i - 1]["gen"]$
            \State $\textit{projections.append}((\textit{start\_aoi}, 1))$ \Comment{+1 marks the begin of the projection}
            \State $\textit{projections.append}((\textit{end\_aoi}, -1))$ \Comment{-1 marks the end of the projection}
            \State $\textit{extension} \gets \textit{extension} + (\textit{end\_aoi} - \textit{start\_aoi})$
        \EndFor

        \State $\textit{projections.sort}(\text{key} \gets x: x[0])$ \Comment{Sort list of tuples using the second element as key}

        \State $\textit{weight} \gets 0$
        \State $\textit{curr\_ext} \gets 0$
        \State $\textit{start} \gets \text{-1}$

        \For{$\textit{projection} \text{ in } \textit{projections}$}
            \If{$\textit{start} \neq -1$}
                \State $\textit{region} \gets \textit{projection[0]} - \textit{start}$ \Comment{Region length}
                \If{$\textit{curr\_ext} + \textit{region} \times \textit{weight} \geq \textit{extension} / 2$}
                    \State \textbf{return} $\textit{start} + (\textit{extension} / 2 - \textit{curr\_ext})$
                \EndIf
                \State $\textit{curr\_ext} \gets \textit{curr\_ext} + \textit{region} \times \textit{weight}$
            \EndIf
            \State $\textit{weight} \gets \textit{weight} + \textit{projection[1]}$ \Comment{Weight is increased/decreased by 1}
            \State $\textit{start} \gets \textit{projection[0]}$ \Comment{Start of new region on projection axis}
        \EndFor
    \EndFunction
\end{algorithmic}
\end{algorithm}

\subsection{Results}
The tested configurations produced a considerable amount of data, that required many hours to be collected. The principal data collected during the experiments are:
\begin{itemize}
    \item \textbf{Message timestamps}, for each message published the subscriber saved both generation and reception timestamps for the \acrshort{aoi} computation.
    \item \textbf{Energy traces}, the energy required by each configuration has been traced by the power monitor as in the first experiment campaign.
    \item \textbf{Metrics on device}, some metrics have been collected on the device side before and after the execution of the code under test, in particular metrics about the quality of the cellular network and the estimated precision of the clock synchronization with the laptop, according to the \acrshort{ntp} protocol.
\end{itemize}

A lot of information has been extracted from this data, which will be reported in the following analyzing a few at a time to focus on the highlights of each. For clarity, the description of the results is then divided into subsections, separating the configurations that add more parameters to take into consideration, similar to the approach already adopted for the first results reported in this thesis.

Before proceeding with the analysis is worth introducing an instrument extensively used to visualize the results achieved both in terms of energy and \acrshort{aoi}. The two metrics, as already specified, are considered together for the energy-constrained nature of the \acrshort{iot} devices, but this introduces additional complexity in the analysis because the objective is to optimize both, but they have a trade-off to be resolved, as will be shown below. Therefore, a possibility is to aggregate the metrics and provide a single result to determine the goodness of a configuration. A simple and effective solution for the aggregation could be a linear combination, assigning a different weight to the metrics, based on their importance. The weights could be normalized, choosing in the zero-one range so that the sum one is one. The underlying problem is that the importance of the metrics is a system-related parameter, i.e. it varies by system, and only the designer can determine the importance of his system. For example, in a system that must take action in response to some detected event, it may be critical to make the decision based on the freshest data, while other systems may prefer to minimize energy consumption at the cost of having less fresh information. The best method for presenting the results is to provide the designer with a tool that shows all possible optimal solutions and leaves it up to him to determine which of those presented is the most suitable configuration for the system. 

The tool that perfectly matches the above requirements is the Pareto front, built up by a set of Pareto efficiencies. Pareto efficiency is a concept introduced by the Italian economist and engineer Vilfredo Pareto and states that given a set of resources an allocation is efficient if is not possible to improve the condition of one individual without worsening those of another, i.e. Pareto improvements are not available. This concept can also be applied in multi-objective optimization when there is no feasible solution that minimizes all objective functions simultaneously. Let us consider a set of points in the plane whose coordinates represent \acrshort{aoi} and energy, respectively, each associated with a particular configuration. The Pareto efficient solutions are those for which one metric cannot be improved without worsening the other. The sub-set of Pareto efficient solutions represents the Pareto front on which a designer can choose the solution to adopt, considering possible constraints of the system in terms of \acrshort{aoi} and energy. The choice can be considered as an a-posteriori assignment of weights to the metrics, based on the knowledge of the considered system. The points having both coordinates worse than other points are referred to as Pareto-dominated and the associated configuration doesn't provide an optimal choice for any system, thus they can be discarded. An example of the Pareto front is reported in \ref{fig:pareto-example}.
\begin{figure}
    \centering
    \includegraphics[width=.85\columnwidth]{images/aoi/pareto_front_example.pdf}
    \caption{Example of Pareto Front}
    \label{fig:pareto-example}
\end{figure}

\subsubsection{Base configuration}
The first set of experiments was carried out by fixing the payload to 128 bytes, the delay to zero and the available cores to one. Considering the remaining parameters, the number of experiments to be performed is given by the cartesian product between 11 rates, 2 transport protocols and 4 queue management policies, thus a total of 88 configurations. For each configuration it is possible to plot the time evolution of the \acrshort{aoi}, from which many more graphs and statistics can be extracted, but in order not to overload the exposition of results with an excessive number of plots only the most significant ones will be reported, ignoring those that do not add any other relevant information than the selected ones. In any case, all graphs can be found within the repository containing the script for running and analyzing experiments \cite{otii-automation}. 

The first configurations analysed have the lowest rate, i.e. one message published each second. The rate doesn't require a reasonably heavy computation to justify a behaviour different to the one expected for the entire duration of the experiment. It thus is confirmed by observing the \ref{fig:time-quic-128B-D0-Q16-R1}, reporting the associated time evolution. The other parameters of the reported configuration are \acrshort{quic} as transport protocol and FIFO-16 as queuing policy, but they are not so relevant because any possible combination with rate one produces a similar result. Looking in more detail at the figure, the shape of time evolution is exactly the one from theory, with the sawtooth swinging from the baseline, given approximately by the one-way delay of the network, to a maximum of around 1 second, i.e. the period elapsed between two message publishing. Also, the mean value is plotted, the red dashed line, and it is around 550ms. The value is consistent with what might be expected because it is positioned roughly at the midpoint between the average maximum and minimum of the series.  

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/aoi_time_evolution_quic_128B_D0_Q16_R1.pdf}
    \caption{\acrshort{aoi} time evolution for 128B, Quic, FIFO 16, Rate 1}
    \label{fig:time-quic-128B-D0-Q16-R1}
\end{figure}

The \acrshort{aoi} time evolution is still quite stable, except for a few spikes, also for the rates 10, 100 and 1000 since the load to be handled is still moderate. The rate increase produces a dramatic improvement in terms of mean \acrshort{aoi}, with a reduction of 83\% from 1 to 10, 25\% from 10 to 100 and 20\% from 100 to 1000, for the \acrshort{quic}, FIFO-16 configuration. The same applies also to the other configurations, even if due to the noisy nature of the experimental data some configurations may present a slight rise of the mean \acrshort{aoi} from rate 10 to rate 100. The mentioned configuration's time evolution and mean value, for the rate 1000, is reported in \ref{fig:time-quic-128B-D0-Q16-R1000}.
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/aoi_time_evolution_quic_128B_D0_Q16_R1000.pdf}
    \caption{\acrshort{aoi} time evolution for 128B, Quic, FIFO 16, Rate 1000}
    \label{fig:time-quic-128B-D0-Q16-R1000}
\end{figure}

The decrease in the mean \acrshort{aoi} encounters a limit from rate 1000 onwards. Most of the configurations show an increase in the mean \acrshort{aoi} going from a rate of 1000 to one of 2000, but a closer inspection shows that contrary to the time evolutions analysed so far, those with higher rates are characterised by the presence of some very high peaks, associated with an \acrshort{aoi} in the order of magnitude of seconds. The peaks enclose a large area below them and therefore the mean value, recalling that is computed employing the integral operator, tends to increase considerably. The origin of peaks can be reasonably attributed to transient adverse network conditions, typical of a wireless connection such as a cellular one. This phenomenon is evident in \ref{fig:time-quic-128B-D0-Q16-R2000}, reporting the time evolution for the rate 2000 in the same configuration reported till now. 
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/aoi_time_evolution_quic_128B_D0_Q16_R2000.pdf}
    \caption{\acrshort{aoi} time evolution for 128B, Quic, FIFO 16, Rate 2000}
    \label{fig:time-quic-128B-D0-Q16-R2000}
\end{figure}

Focusing on the peaks it is possible to observe a different shape between the rising and falling edges:
\begin{itemize}
    \item \textbf{Rising edge}, the rising is sharp, with none or few saw teeth, which means that for the entire period, the messages are not delivered to the subscriber.
    \item \textbf{Falling edge}, the falling is very jagged due to the presence of many small saw teeth, an indication of the close arrival of many messages.
\end{itemize}

What can be deduced is that the missed delivery of messages causes the \acrshort{aoi} to increase steeply, up to an inversion of trend after which all undelivered messages are received in a short time interval re-establishing an \acrshort{aoi} in the expected range. The assumption of transient network conditions perfectly matches the behaviour deduced from the peak shape analysis, because when network conditions are adverse, messages do not reach the broker, delaying the delivery to the subscriber. Note that given the large number of parameters involved, many of which are not the subject of analysis, adverse network conditions may not be the direct cause of peak generation. However, it is still reasonable to consider this transient situation at least as the trigger for other phenomena that cause messages to fail. For example, the congestion control mechanism may come into play, which considers the missed reception of acknowledgements, often due to network conditions, as congestion and thus drastically reduces the transmitting rate. A zoom on the second peak, i.e. the one between forty and fifty seconds, is shown in \ref{fig:aoi-zoom-peak}.
\begin{figure}
    \centering
    \includegraphics[width=0.80\columnwidth]{images/aoi/zoom_peak.pdf}
    \caption{Focus on \acrshort{aoi} peak}
    \label{fig:aoi-zoom-peak}
\end{figure}

As anticipated the mean value is negatively affected by the presence of sporadic peaks associated with transient network conditions. However, for a fair comparison between different configurations such peaks should be filtered because related to random external factors on which it is not possible to operate. The introduction of the median allows exactly the aggregation of time evolution data filtering out the extreme values. In the latter \acrshort{aoi} time evolution plot, \ref{fig:time-quic-128B-D0-Q16-R2000}, the orange dashed line is the median value, computed according to the method described in Algorithm \ref{alg:median}. The height of the orange line is greater than the red one, i.e. the median value results in a smaller value than the mean value. The difference between the two metrics is compatible with the definition of the two because the mean tends to assume a higher value due to the peaks, while the median that is more robust to isolated peaks assumes a lower value. The mean and median values of the configuration reported so far can be found in \ref{tab:mean-vs-median}. From the table, it is possible to appreciate the progressive difference between the two metrics, the greater the rate and thus the greater the probability that a transient network event can cause sudden increases in the \acrshort{aoi}. 
\begin{table}
  \centering
  \caption{Difference between mean and median values for \acrshort{quic}, FIFO-16 configurations}
  \label{tab:mean-vs-median}
  \begin{tabular}{lrrr}
    \toprule\toprule
    \textbf{Configuration} & \textbf{Mean [ms]} & \textbf{Median [ms]} & \textbf{Difference [ms]} \\
    \toprule
    Rate 1 & 551.12 & 551.13 & - \\
    \midrule[0pt]
    Rate 10 & 95.60 & 93.28 & 2.32\\
    \midrule[0pt]
    Rate 100 & 72.03 & 69.16 & 2.87\\
    \midrule[0pt]
    Rate 1000 & 50.08 & 45.15 & 4.93\\
    \midrule[0pt]
    Rate 2000 & 57.98 & 43.66 & 14.32\\
    \bottomrule
  \end{tabular}
\end{table}

A final observation about the data presented so far is that the minimum \acrshort{aoi} is around 40 ms. This is not a random value, it is a lower bound given by the experimental setup built to carry out the experiments. Recalling the \ref{tab:net_stats}, the \acrshort{rtt} in the network segment \acrshort{rpi}-server is about 80 ms and assuming a symmetric path it is reasonable to consider the one-way delay the half of \acrshort{rtt}, i.e. 40 ms. This consideration, together with the fact that the second network segment, connecting the server with the subscriber, is almost negligible since both devices are in the same network, determines the minimum \acrshort{aoi} that can be experienced in this setup.

Before moving to the aggregate results of the configuration with higher rates is necessary to point out a limit of the median value, the one that will be considered for the remaining data. As already highlighted the introduction of the median allows to filter out of sporadic peaks that are related to random external phenomena, but even if for comparison purposes this approach is necessary the risk is to hide some aspects in the final evaluation. Observing some time evolution associated with the higher rates the problem is evident because when the system is overloaded the same conditions that would have generated an isolated peak cause far more prolonged worsening of the \acrshort{aoi}, that can last for a significant amount of time. This phenomenon is completely hidden aggregating via the median, as reported in \ref{fig:median-problem} for the configuration Quic, FIFO-16 and rate 8000. From a certain point of view, it's correct to filter out the entire transient period because as originates from an external factor, but analysing the various configurations the ones that present the prolonged peaks are all associated with high rates and FIFO-1/16 queuing policy, so it's reasonable to state that some configurations are more robust against transient adverse network conditions. Robustness is an appreciable property because transient network degradation is a real problem to deal with, and some applications may be sensitive to maximum \acrshort{aoi}, also referred to as peak \acrshort{aoi}. In this thesis, the peak \acrshort{aoi} is not taken as the reference metric, but it is worth noting that by acting on the queuing mechanism it might be possible to tune the system to optimize this metric as well.
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/aoi_time_evolution_quic_128B_D0_Q16_R8000.pdf}
    \caption{Median problem}
    \label{fig:median-problem}
\end{figure}

Moving the analysis to rates above 2000, the \acrshort{aoi} stops decreasing permanently, but since the lowest possible value has already been reached, this result is quite obvious. A more interesting observation is that from rate 3000 onward, the first difference between queue management policies can be appreciated:
\begin{itemize}
    \item \textbf{FIFO}, the time evolution \acrshort{aoi} is increasingly unstable as the transmission rate increases, worsening the median value. 
    \item \textbf{Head-Drop}, the time evolution \acrshort{aoi} is much more stable and the median value is stationary around the minimum value as the rate increases.
\end{itemize}

Several factors determine this difference, but the key point is that in the FIFO policy messages are enqueued when the system is not able to process them, while in the head-drop policy the messages that can't be handled before the next generation will be overwritten, in such a way that only messages containing the most recent information will be transmitted, thus minimizing the \acrshort{aoi} at the subscriber side. Reasoning at a high level the two queuing policies show their differences starting from high rates when the system load increases up to a point for which the generation of messages requires more time than the generation period. In the FIFO policy, this situation leads to message queuing that negatively affects the \acrshort{aoi}, whereas in the drop policy, the messages are overwritten. In \ref{fig:drop-fifo-quic-line} the line plot reports the median \acrshort{aoi} trend over the nominal rates for the \acrshort{quic} configurations. The rates up to 1000 are not included in the graph to guarantee better readability, avoiding a flattening of the lines due to the scale of the y-axis. The lines tend to intersect several times, but what needs to be inferred is the different trend between the two queuing policies, with FIFO tending to worsen and head-drop remaining stable. The fluctuations are due to the experimental nature of the data and the use of a cellular network that cannot guarantee perfect stability while running all configurations. Note that the same applies for the \acrshort{tls} configurations, and although the fluctuations are more severe the trend still holds. Finally, it's worth recalling that from the literature the head-drop policy, which can be considered as a LIFO policy, is generally the optimal one to minimize the \acrshort{aoi}.
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{images/aoi/quic_median_aoi_over_rate.pdf}
    \caption{Median \acrshort{aoi} over rate for Head-Drop and FIFO policies}
    \label{fig:drop-fifo-quic-line}
\end{figure}

Completed an overview about the \acrshort{aoi} trend over the rates and observed the time evolutions the analysis can move on to the difference between the various configurations, particularly the differences between the transport protocols and the queuing policies. A major difference between queuing policies has already emerged, but it is possible to go deeper into the analysis reporting other consequences descending directly by the queuing mechanism, i.e. the real transmission rate supported by the system. The real rate is measured at the subscriber side, as the reception rate that computed as the inverse of the mean interarrival time, i.e. time elapsed between two message arrivals. As already highlighted many times, the effects introduced by the second network segment are almost negligible to the ones of the segment publisher-broker, thus the reception rate is dominated by the transmission rate supported by the publisher on the \acrshort{rpi}. 

Moreover, comparing the real rate with the generation rate at the publisher, computed with the same procedure, shows that they are very close in the case of the FIFO policy. Considering that the generation of messages stops only when the queue is full, i.e. the task dedicated to transmitting data is not able to transmit all messages generated, \ref{sec:client-tool}, the latter will adapt to the sending rate. Given the equivalence between generation and reception rate, the assumption of employing the reception rate for the following analysis is validated. Note that the generation and reception rates are easily extracted from the data collected because of the recording of timestamps for the \acrshort{aoi} computation, so they come for free without the need to add additional probes in the developed code. 

Before going on with the analysis of the real rate it's necessary to point out that the above reasoning applies only to the FIFO queuing policy since the head-drop one doesn't involve a fixed length queue, but a buffer that can be overwritten, so the generation rate will be fixed to the nominal one, unless there are sufficient computing resources on the \acrshort{rpi}, without adapting to the transmission rate. 

The above-mentioned difference regarding the real rate is shown in \ref{fig:real-nominal-rate}, in which the x-axis reports the nominal rate, while the y-axis the real rate. Each colour is associated with a different queuing policy, the solid lines are \acrshort{quic} configurations whereas the dashed lines are \acrshort{tls} ones. In the ideal case, the nominal rate equals the real one so the associated line is a bisector, but in situation depicted in the graph is not ideal. The only configuration that allows to reach the highest rate is \acrshort{quic}, FIFO-1024 while the counterpart \acrshort{tls} is slightly below. The same applies to FIFO-16 but in this case, the upper bound is around 7000 for both protocols, with \acrshort{quic} reaching again a slightly higher rate than \acrshort{tls}. Limiting the analysis of these two queuing policies the conclusion could be that \acrshort{quic} behaves a little better in terms of reachable transmission rate given the producer-consumer pattern implemented in the client-tool. This result partially mirrors the one presented for the first experiment campaign, \ref{chap:energy}, in which even if the results were in many cases very close the feeling was that \acrshort{quic} could guarantee a faster transmission that allowed for lower energy consumption in some cases. The precedent scenario was quite different because the connection establishment had a non-marginal impact since only one message was published, so the idea was that the lighter mechanism of \acrshort{quic} was primarily responsible for the difference. However, the difference is still valid in this scenario, where the connection establishment loses centrality due to the high number of messages published on the same connection, reinforcing the feeling that \acrshort{quic} may guarantee a faster transmission. All these considerations are swept away once observing the real rate for the FIFO-1 configurations. Both configurations are not able to approach the highest rate, but the \acrshort{tls} can reach a real rate of about 5000, while the \acrshort{quic} one stops just above 2000. After this observation is clear that adding space in the queue allows reaching a higher rate. Intuitively, the explanation for this result is that the presence of a queue allows the messages to be queued without reducing the generation rate, allowing the consumer task to send those messages at the maximum supported rate without blocking waiting for new messages. The queue maximizes the utilization of available resources on the \acrshort{rpi}, particularly by taking full advantage of the available bandwidth. From a deeper analysis, supported through the collection of network traces via the tcpdump tool, the difference between rates appears to be due to a different transport-level aggregation factor for the various configurations. Specifically, when the application queue allows more than one message to be inserted, the transport layer can saturate the transmitted segment thus optimizing network resource utilization. Conversely, when the queue does not allow more than one message to be stored, the transport layer is unable to perform any aggregation, sending a segment of reduced size each time, and introducing a non-negligible overhead. Regarding the difference between the two FIFO-1 configurations, the cause seems to be a more aggressive aggregation performed by the \acrshort{tls} protocol, inherited by \acrshort{tcp}, by Nagle's algorithm. This algorithm is not based on timeout, after which the segment is sent, but on the presence or absence of pending acknowledgement referring to previous packets. Following Nagle's algorithm, a segment can be sent out only if one of two conditions is met:
\begin{itemize}
    \item There aren't pending acknowledgements at the transport level
    \item The segment is filled, it is worth recalling that the \acrshort{mss}, which rules the maximum size for the transport layer packet is established in the initial handshake and for the experimental setup is 1360 bytes.
\end{itemize}
The presence of such a mechanism determines a greater aggregation than \acrshort{quic}, also when the application queue has only one position. The intuition about Nagle's algorithm is confirmed by observing the maximum achievable rate, and the aggregation level, disabling it via a simple configuration of the socket opened by the client tool. The \ref{tab:througput-aggegation} reports the number of transport segments sent by the publisher toward the subscriber for a \acrshort{fifo}-1 configuration with a nominal rate of 3000 messages per second, the mode of application messages inside a single segment along with the number of occurrences, and the throughput achieved, i.e. the real rate measured. Note that the maximum achievable rate disabling Nagle's algorithm is below 3000 messages per second, while the standard \acrshort{tls} can approach up to 5000 messages per second. A test with a higher rate would better highlight the difference between the two versions, however, it would require a non-negligible overhead in the collection of the network traces. The data reported shows that by disabling Nagle's algorithm the aggregation is substantially prevented and the maximum achievable rate decreases. However, even if the difference between \acrshort{quic} and \acrshort{tls} shrinks disabling Nagle's algorithm a deeper analysis should be carried out to shed light on the encountered behaviour. 
\begin{table}
  \centering
  \caption{Aggregation impact on throughput}
  \label{tab:througput-aggegation}
  \begin{tabular}{lrrr}
    \toprule\toprule
    \textbf{Transport Protocol} & \textbf{\# Packets} & \textbf{Aggregation} & \textbf{Throughput} \\
    \toprule
    \acrshort{tls} & 22029 & 8 \small{(13807)}, 9 \small{(7365)} & 3000 msg/s \\
    \midrule[0pt]
    \acrshort{tls} (Nagle disabled) & 177167 & 1 & 2752 msg/s \\
    \midrule[0pt]
    \acrshort{quic} & 179484 & 1 & 1990 msg/s \\
    \midrule[0pt]
    \bottomrule
  \end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{images/aoi/real_vs_nominal_rate.pdf}
    \caption{Real and Nominal rate for 128B}
    \label{fig:real-nominal-rate}
\end{figure}
Regarding the comparison between transport protocols, the analysis must be broken down by rate ranges because there is no general conclusion that can be applied in absolute terms. The regions identified by rate ranges are three:
\begin{enumerate}
    \item \textbf{Slow rates}, includes the two slowest rates, i.e. 1 and 10 messages per second.
    \item \textbf{Medium rates}, includes the rates spanning from 100 to 4000, thus including the lower points of the \acrshort{aoi} curves.
    \item \textbf{High rates}, include the highest rates, from 5000 to 8000, for which the heavy computational load tends to increase the noise in the collected data.
\end{enumerate}

In the first region, \ref{fig:median-rate-slow}, the curves associated with the different configurations, recalling that only transport protocol and queue policy are not fixed, are very close. There are no one or more dominant configurations, even if, mainly for the rate 10, the \acrshort{tls} configurations seem to provide slightly better results in terms of \acrshort{aoi}. The only configuration that does not reflect the given description is \acrshort{quic}, FIFO-1024, which is characterized by a significantly higher median \acrshort{aoi} for both rates. There is no particular reason to explain the difference, in fact with these transmission rate values the other parameters of the configurations have no appreciable impact. The explanation for this odd behaviour is obtained by looking at the bad synchronization accuracy recorded during the configurations running. The first configuration, rate 1, suffered from a synchronization offset in the order of one hundred milliseconds, which raised the median value of such quantity, while for the second one, the offset was in the order of 60 milliseconds, increasing again the aggregated value reported in the graph. Note that the synchronization referred to is between the \acrshort{rpi} and the laptop, thus the publisher and subscriber from the \acrshort{mqtt} point of view.
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{images/aoi/median_aoi_over_rate_ragion_0.pdf}
    \caption{Median \acrshort{aoi} over rate (slow rates)}
    \label{fig:median-rate-slow}
\end{figure}

The second region, \ref{fig:median-rate-medium}, is characterized by the knee of the majority of curves that reach their minimum value for the reported rates. The difference in behaviour between queue policies has already been pointed out, but the difference between transport protocols deserves equal attention. The \acrshort{tls} configurations, the dashed lines, are located above the \acrshort{quic} configurations, solid lines, for all points except one point in the FIFO-16 series, which is affected by heavy fluctuations. This trend is glaring in the initial part of the graph, for the rates 100 and 1000, where all \acrshort{quic} configurations lie down the \acrshort{tls} ones, but focusing on the comparison between the same queue policy the trend still holds for the other points. However, must be highlighted that the difference tends to shrink moving toward higher rates, up to 4000 for which the same queue policy configurations are very close. Although taking into account the noisy nature of data, \acrshort{quic} for this range of rates seems to guarantee better results in terms of \acrshort{aoi}. Moreover, focusing on FIFO-1 configurations is interesting to note that despite the marked difference in the maximum reachable rate between the two transport protocols, the \acrshort{aoi} doesn't reflect this gap. At first glance, this might seem not possible, but by reasoning about the computational model the doubts can be cleared. In particular, having only one position in the queue between producer and consumer leads to the former getting blocked every time the consumer fails to empty the queue in time, and although this results in a reduction of the achievable throughput the fact that the newly produced message has nothing ahead limits the delay experienced and thus the \acrshort{aoi}.
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{images/aoi/median_aoi_over_rate_ragion_1.pdf}
    \caption{Median \acrshort{aoi} over rate (medium rates)}
    \label{fig:median-rate-medium}
\end{figure}

Finally, in the third region, \ref{fig:median-rate-high}, are reported the highest rates, for which there is no clear trend, apart from the difference between drop and FIFO policies already described. Focusing on the differences between transport protocols there are many intersections between lines, even for the same queue lengths. There is no reason why intersections should be a systematic phenomenon related to configurations and the lines are often quite close, so it's legit to consider such fluctuation as noise in the data, exacerbated by the heavy load in the system given by the high transmission rates.  
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{images/aoi/median_aoi_over_rate_ragion_2.pdf}
    \caption{Median \acrshort{aoi} over rate (high rates)}
    \label{fig:median-rate-high}
\end{figure}
Please note that the analysis of the three regions and associated graphics was carried out taking into account the nominal rates, but the actual rates are lower for certain configurations as already pointed out.

Until now only the \acrshort{aoi} has been considered, but the initial statement was that experiments should aim to conduct a combined study with the energy. So, before presenting the combined results an overview from the energy side is given, in a similar manner to what is already done with the \acrshort{aoi}. Recalling the first campaign of experiments, energy results were presented by aggregating for the various repetitions the energy required to publish a message with a given configuration. In these experiments, the energy of the total time window is considered, regardless of the individual request, for which it would be rather complex to isolate the associated portion of energy due to the possible high transmission rate. Having only one repetition, as for the \acrshort{aoi} may involve some limitation from a statistical point of view, but the presence of a time window rather than a single request guarantees a more robust result even without repeating the experiment many times. The real problem is that, despite the nominal duration of the time window being fixed for all configurations, the actual duration is established by the real rate reached during the experiment. The number of messages to be published is determined by considering the nominal rate, so if this rate is not supported the experiment will take longer to complete all the expected transmissions. In principle, this is not a problem but the experiments aim to measure the \acrshort{aoi} and energy consumed to achieve such \acrshort{aoi}. The method adopted to present the data without ambiguity on how to interpret the results is to normalise the energy considering the time, i.e. dividing the total energy by the actual time of the experiment. This calculus,  equation \ref{eq:power}, is simply the expression for the average power, i.e. energy spent in the unit of time. 

\begin{equation}
    \label{eq:power}
    P_{avg} = \genfrac{}{}{1pt}{}{Energy}{Time}\:\genfrac{}{}{0pt}{}{(J)}{(s)}
\end{equation}
The method is validated by observing that sixty seconds are sufficient to reach a stationary situation, as can be deduced by looking at any time evolution graph, so it is possible to say that the power will take the same value regardless of the time window considered and consequently the actual time taken to complete the transmission of all messages.

The energy results for the different configurations can be presented after the initial premise. The first result to be reported is the trend of average power over the nominal rate. As shown in \ref{fig:power-over-nominal-rate}, the trend is almost vertical for the first few rates, due to a significant increase in the required power going from rate 1 to 10 and from rate 10 to 100 which are relatively close. After this initial increase, the power, as expected, continues rising with the rate but with a slower slope. This trend is valid for all configurations, considering both transport protocols and queuing policies, at least up to the rate of 2000. From such a rate onward the drop policy stops increasing and the same applies for FIFO-1, but only in the \acrshort{quic} configuration. Moreover, also the FIFO-1 \acrshort{tls} encounters an upper bound around the rate of 5000. The remaining configurations, even if subjected to some fluctuations, present a quite evident increasing trend up to the maximum rate. The overview of the trend and the points after which some configurations don't present an increasing average power suggest that the power consumption is dominated by the transmission rate, thus once the maximum rate for a configuration is met further increases in the nominal rate won't produce any significant variation in terms of average power. In support of this conclusion, another experiment conducted with two CPU cores enabled will be presented below. 
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{images/aoi/power_over_nominal_rate.pdf}
    \caption{Average power over nominal rate}
    \label{fig:power-over-nominal-rate}
\end{figure}
Regarding the comparison of transport protocols, excluding the first two rates for which no obvious trend is visible, two regions, separated by the rate of 2000 can be identified. The first one includes rates from 100 up to 2000 and, as reported in \ref{fig:power-over-low-real-rate}, there is a clear difference between \acrshort{quic} and \acrshort{tls} configurations, with the latter characterized by lower energy consumption regardless of the queuing policy, except for the last point for FIFO-1024, which is still lower comparing the two curves associated with that policy. The power difference is mainly due to the transport protocol adopted, while the contribution of the queuing policy, in this region, is practically negligible. Another observation in favour of this statement is that by focusing on the two groups of lines separately there is no ordering for queuing policy configurations inside the group. Let's now focus on the second region. \ref{fig:power_over_high_true_rate} includes the rates above 2000, so only a subset of configurations are considered, i.e. the ones able to exceed the threshold of 2000 messages per second. Those configurations are FIFO-1024, FIFO-16 and FIFO-1 only in the \acrshort{tls} version. The configurations are no longer as well separated as the first rates: for the FIFO-16 configurations, the comparison between transport protocols produces the same result, i.e. \acrshort{quic} requires more power, but for FIFO-1024 the lines intersect multiple times, so it is difficult to draw some conclusions. The intersections for FIFO-1024 may derive from the fluctuations of the experimental data and not from underlying phenomena, so the most appropriate conclusion is that for that queuing policy the two transport protocols guarantee very similar results. This conclusion fits well also for the trend in the first region, observing that yet for the rate 2000, the lines appear quite close. The other aspect that deserves attention is that the FIFO-16 configuration presents the highest power consumption in the second region. It is not easy to find a clear explanation for this result, but it is reasonable to attribute this higher energy consumption to less efficient utilization of network resources. Recalling the analysis on the aggregation of messages at transport protocol having a smaller queue length allows for a less aggressive aggregation, requiring a higher number of transmitted packets with smaller size, resulting in worse exploitation of available network resources. A final consideration about the second region is that the queuing policy, contrary to the first region, assumes a significant role in power consumption, while the difference due to transport protocol tends to disappear. Please note that \ref{fig:power-over-real-rate} reports the actual rate on the x-axis, contrary to the other graph for which the nominal rate was employed, because the actual rate, rather than the nominal, is the main factor that determines the power consumption.
\begin{figure}
    \centering
    \begin{subfigure}{0.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/aoi/power_over_true_rate_region_1.pdf}
        \caption{Low rates region} 
        \label{fig:power-over-low-real-rate}
    \end{subfigure}%
    \begin{subfigure}{0.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/aoi/power_over_true_rate_region_2.pdf}
        \caption{High rates region} 
        \label{fig:power_over_high_true_rate}
    \end{subfigure}%
    \caption{Average power over real rate}
    \label{fig:power-over-real-rate}
\end{figure}

\subsubsubsection{Pareto Efficiency}
The \acrshort{aoi} and energy results can be combined building a Pareto front, as already described above. The Pareto front reports average power on the y-axis and \acrshort{aoi} on the x-axis, each point is associated with a different configuration in terms of rate, queuing policy and transport protocol. The queuing policies, so far jointly analysed, fulfil different requirements as already pointed out, so two different Pareto fronts will be reported, one for the FIFO policy and one for the head-drop one. To recognize the rates, the nominal value is reported near the corresponding point in abbreviated form to save space, replacing the thousands with the letter "K".

The Pareto front for FIFO queuing policy is reported in \ref{fig:paret-front-fifo}, the dominated points are not present to avoid confusion. The first observation concerns the rates that appear in the front, which do not exceed 2000 messages per second. The adoption of high transmission rates does not guarantee advantages for either power consumption or \acrshort{aoi}. This result is quite important because shows that, even if high rates can be reached by employing long queues they do not lead to benefits in the system that will result in overload, increasing drastically the power consumption and not improving the \acrshort{aoi}. The worsening of \acrshort{aoi} at high rates at first glance may not be obvious, but once network resources are saturated packets are queued in the system, both at the application level and in the underlying layers, increasing the delay experienced by messages that will be delivered already aged. Remaining on the analysis of rates in the front is clear the trade-off between power consumption and the \acrshort{aoi} for the rates of the points belonging to the front. Lower rates guarantee a smaller average power due to the low utilization of the system, at the cost of a large \acrshort{aoi} dominated by the fact that the messages are spaced over a large period. Higher rates contrary allow for reduction of the \acrshort{aoi} up to the lower bound given by the one-way delay, but at the cost of increasing the system utilization and thus the average power consumption. 
\begin{figure}
    \centering
    \includegraphics[width=.85\columnwidth]{images/aoi/pareto_front_fifo.pdf}
    \caption{Pareto front for FIFO configurations}
    \label{fig:paret-front-fifo}
\end{figure}
The figure shown suffers from the fact that by going from rate 1 to rate 10 the \acrshort{aoi} improves dramatically. For this reason, a zoom of the left part is reported in \ref{fig:pareto-front-fifo-zoom}. In this figure, apart from the already mentioned trend for the rates, is possible to appreciate another result, i.e. the points on the left-extreme are all related to \acrshort{quic} configurations that highlight the capability of such protocol to guarantee a lower \acrshort{aoi}. The high density of points in the left extreme also shows that once approaching the lower bound further improvement, even if small in terms of percentage, requires a significant increment in the power consumption. Regarding the comparison between queue length the arrangement of the points in the front does not suggest any evident trend, moreover, the noise that characterises the experimental measurements does not allow for drawing any clear conclusion.   
\begin{figure}
    \centering
    \includegraphics[width=.85\columnwidth]{images/aoi/pareto_front_fifo_zoom.pdf}
    \caption{Zoom of Pareto front for FIFO configurations}
    \label{fig:pareto-front-fifo-zoom}
\end{figure}

Moving to the Pareto front for the head-drop queuing policy some differences deserve to be highlighted. First of all, the front reported in \ref{fig:pareto-front-drop-zoom} is zoomed, cutting off rate 1 for readability reasons, as already done for the FIFO one. The trend that can be observed is initially similar to the FIFO configuration, characterised by a trade-off between \acrshort{aoi} and power consumption. However, once the transmission rate reaches values around 2000, the drop policy can further improve the \acrshort{aoi} by adopting higher nominal rates. In the front, rates appear up to the maximum, i.e., 8000 messages per second. Even if every nominal rate above 2000, or even less, results in the same real transmission rate, keeping the power consumption limited, the \acrshort{aoi} continues to slightly decrease because of the possibility of overwriting the buffer, which permits the generation rate to equal the nominal one, independently from the transmission rate. So, the result is that each time the buffer is emptied the new message will be written according to the nominal rate, having each time the freshest information to be sent. In the FIFO case, even if the producer stops generating new messages, those stuck in the queue will age, resulting in the transmission of older information. This is the reason why the head-drop policy is the optimal one for the \acrshort{aoi}, but once again is worth recalling that by adopting such a policy the system should admit message loss due to the overwriting of the buffer. Finally, the comparison between transport protocols produces the same result, i.e. \acrshort{quic} allows for better \acrshort{aoi} at the cost of higher energy consumption.
\begin{figure}
    \centering
    \includegraphics[width=.85\columnwidth]{images/aoi/pareto_front_drop_zoom.pdf}
    \caption{Zoom of Pareto front for Head-Drop configurations}
    \label{fig:pareto-front-drop-zoom}
\end{figure}

\subsubsection{Additional delay}
The results of the first experiment campaign showed interesting results about the comparison between \acrshort{tls} and \acrshort{quic} adding extra delays, so also for this new scenario configurations with artificial delay are been tested. In particular, the values considered are the same, from 20 to 80 milliseconds, which are summed to the real delay experienced by the setup. The analysis follows the same path adopted for the results without additional delay and, again to avoid confusion only a small subset of graphs will be reported in the thesis. Moreover, the analysis will focus on the Pareto fronts, one for each delay configuration, to spot any possible variations in the different scenarios.
The first observation is on the \acrshort{aoi} shape, that matches the one expected already extensively described. Focusing on the individual time evolutions for low rates is not very interesting since they have exactly the usual trend already observed in the case without additional delay, with only an upward shift of the entire \acrshort{aoi} function of a value in the order of the set delay. The only valuable remark is on the slowest rate, one message per second, for which the upward shift represents a small percentage of the experienced median \acrshort{aoi}. This is clearly due to the slow rate adopted, which in this configuration is the main responsible for the poor \acrshort{aoi} obtained. So in this particular configuration, although it produces an increase in the metric, it is unlikely to heavily impact the freshness of data. A slight increase in the transmission rate is sufficient to generate a completely different result, attributing a significant impact of the additional delay on the obtained \acrshort{aoi}. Some data confirming this trend are reported in \ref{tab:delay-rate-1} and \ref{tab:delay-rate-10}, from which can be noted the increment in percentage terms compared to the base case without artificial delay. Both tables present the median \acrshort{aoi} for the \acrshort{quic} and FIFO-16 configuration varying the artificial delay. The shift column reports the percentage increment of the median \acrshort{aoi}. The first table refers to rate 1, for which the increases are less than 10 percentage points up to 80 milliseconds delay, for which the shift can no longer be considered negligible. The second relates to rate 10, for which the addition of an extra delay profoundly affects the obtained \acrshort{aoi}, up to almost double the base rate. 
\begin{table}
    \begin{minipage}{.5\linewidth}
    \centering
    \caption{\acrshort{aoi} shift for \acrshort{quic}, FIFO-16, Rate 1}
    \label{tab:delay-rate-1}
	\begin{tabular}{lrr}
		\toprule\toprule
		\multicolumn{1}{c}{\textbf{Delay}} & \multicolumn{1}{c}{\textbf{Median \acrshort{aoi}}} & \multicolumn{1}{c}{\textbf{Shift}} \\
		\midrule
		None & 551.13 & - \\
		\midrule[0pt]
        20 ms & 571.65 & 3.7\% \\
		\midrule[0pt]
		40 ms & 587.49 & 6.6\% \\
        \midrule[0pt]
		60 ms & 602.93 & 9.4\% \\
        \midrule[0pt]
		80 ms & 708.08 & 28.5\% \\
        \bottomrule
	\end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
    \centering
    \caption{\acrshort{aoi} shift for \acrshort{quic}, FIFO-16, Rate 10}
    \label{tab:delay-rate-10}
	\begin{tabular}{lrr}
		\toprule\toprule
		\multicolumn{1}{c}{\textbf{Delay}} & \multicolumn{1}{c}{\textbf{Median \acrshort{aoi}}} & \multicolumn{1}{c}{\textbf{Shift}} \\
		\midrule
		None & 93.28 & - \\
		\midrule[0pt]
        20 ms & 107.17 & 14.9\% \\
		\midrule[0pt]
		40 ms & 123.72 & 32.6\% \\
        \midrule[0pt]
		60 ms & 143.62 & 54.0\% \\
        \midrule[0pt]
		80 ms & 178.65 & 91.5\% \\
		\bottomrule
	\end{tabular}
    \end{minipage}
\end{table}
The only odd behaviour in the tables concerns the configuration with 80 milliseconds delay for rate 1, which is considerably higher than expected. A deeper analysis is required to discriminate between an underlying phenomenon or a simple distortion of the data due to adverse network conditions. The latter seems to play a role because, as already done for some strange results in \ref{chap:energy}, some network quality signal indicators are not very good. In particular, the \acrshort{rsrq} an indicator that sums up both on \acrshort{rssi} and \acrshort{rsrp}, shows a value before and after the configuration below -17 DBm, that can be classified as quite scarce. Such value is typically around -15 DBm, however, the signal quality might be not the only cause of the gap.

The effect of the additional delay can be visualized in \ref{fig:aoi-time-evolution-delay-comparison}, reporting the \acrshort{quic}, FIFO-16 configuration for rate 1000 varying the artificial delay. The upward shift can be appreciated moving from left to right, observing the baseline rising of a quantity in the order of the associated delay. This trend is valid for all the configurations, even if for some it may be less evident due to the noisy nature of data.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/aoi_time_evolution_delay_comparison.pdf}
    \caption{Comparison of \acrshort{aoi} time evolution for different delays}
    \label{fig:aoi-time-evolution-delay-comparison}
\end{figure}

Regarding the comparison between queuing policies, the first observation is about the maximum rate achieved by the different configurations. The trend is unchanged varying the delay, i.e. a long queue allows for higher rates to be reached. However, by increasing the delay there is an overall reduction of the maximum rate, mainly for \acrshort{quic}, moving the upper bound to lower values for FIFO-1024 and FIFO-16 configurations while for FIFO-1 and head-drop the highest achievable rate remains constant. This trend can be visualised in \ref{fig:maximum-rate-delay}. The reduction for \acrshort{quic} configurations is such that starting from 40 milliseconds delay is \acrshort{tls} the transport protocol that guarantees a faster transmission rate, contrary to the results obtained so far. The possible causes can be due  to an interaction of multiple aspects:

\begin{itemize}
    \item \textbf{Congestion control}, the congestion control algorithm is the same, Cubic, for both transport protocols, however, the parameters of operation may differ, resulting in different performance when varying the network delay.
    \item \textbf{Flow control}, the advanced flow control mechanism of \acrshort{quic} based on multiple streams is not exploited by the implemented tool, so in this configuration also \acrshort{quic} may suffer from head-of-line blocking problem. 
    \item \textbf{Aggregation}, the aggregation at the transport layer for \acrshort{tls}/\acrshort{tcp} is based on Nagle's algorithm, that for high transmission rates allows for sending only fully sized segments, independent by the network delay, while \acrshort{quic} adopts a blander aggregation mechanism 
    \item \textbf{Kernel optimization}, as already pointed out the Linux kernel on the \acrshort{rpi} doesn't offer optimization for the \acrshort{udp} protocol, such as \acrshort{gso}, potentially reducing the performance of \acrshort{quic}.
\end{itemize}
The mentioned aspects are the primary factors that may justify the inversion trend in the maximum rate for high delay, however, a deeper analysis should be required to better understand the phenomenon.
\begin{figure}
    \centering
    \includegraphics[width=0.85\columnwidth]{images/aoi/max_rate_delay.pdf}
    \caption{Maximum rate for different delays}
    \label{fig:maximum-rate-delay}
\end{figure}

In terms of \acrshort{aoi} and energy consumption, the same considerations roughly apply also adding the delays, both comparing queuing policies and transport protocols. Due to the absence of evident variation, the most effective solution to present the data is to directly report aggregated form, i.e. the Pareto fronts, one for each additional delay. Before analysing the fronts, is worth explaining the reason why each extra delay must be associated with a different Pareto front, instead of summarising all in the same front. The choice is motivated by the fact that each additional delay represents a different scenario within which a different sub-set of configuration may result in the optimal one. The objective of the Pareto front is to assist in finding trade-off between \acrshort{aoi} and energy consumption, starting from the knowledge of the environment in which the system will operate. For this reason, a different Pareto front is required for each additional delay.

The \ref{fig:pareto_front_delay_fifo} reports all the Pareto fronts, including the base one already described above, for the FIFO configurations. The meaning of the colours and the shape of the markers are the same as in the previous graphs although there are more curves to observe separately. To avoid excessive confusion in the graph there are no annotations about the delay associated with the Pareto fronts, taking advantage of the fact that the results obtained are such that the various curves are naturally separated, allowing them to be identified without any specification. Moreover, the fronts have been cut, leaving out the far-right points generated by rate 1, to focus on the most interesting region.
Looking at the Pareto fronts, it is possible to notice that all the considerations valid for the case without additional delay are still valid, i.e. lower rates guarantee a low power consumption, at the cost of higher \acrshort{aoi}, while increasing the rate the opposite applies. Moreover, increasing the rate above 2000 messages per second doesn't guarantee benefits in any scenario. This statement has two exceptions, given by the upper point in the third and fourth curves obtained with a nominal rate respectively of 6000 and 5000 messages per second. This result was unexpected, but focusing on the queuing policies some doubts can be cleared. Both the odd results are obtained for a \acrshort{quic} configuration with FIFO-1 queue, i.e. a configuration that limits its maximum real transmission rate to 2000. For FIFO configurations the generation rate adapts to the transmission one, so it can be considered equal to a configuration having a lower rate, at least from the \acrshort{aoi} point of view. In terms of energy, the additional power required to move from the second highest point in the curve to it represents a significant increment that can be hardly justified by the undetectable improvement in terms of \acrshort{aoi}. Another consideration is about the comparison between \acrshort{quic} and \acrshort{tls}, that for each configuration holds the observation that the first one reaches lower \acrshort{aoi} value, but with a higher power consumption taking the rate fixed. This result originates a quite visible trend, characterised by the shift of the \acrshort{quic} points to the top-right of the curve. This trend was already present in the first Pareto front, but now it is confirmed observing that it is valid for all the reported fronts. Another notable observation is the distance between the first four curves and the last one, which represents the scenario with 80 additional milliseconds delay. The distance is covered both horizontally and vertically, even if the horizontal one is partially due to the extra delay. The dramatic worsening for such delay was already noted analysing the tables about median \acrshort{aoi} shift, \ref{tab:delay-rate-1} and \ref{tab:delay-rate-10}. Looking at the network status the entire experiment suffered from poorer network conditions than the others. Still, it is probably only a factor that jointly with other underlying phenomena produced such a result.

A final remark on the displacement of the queuing policies in the various curves, for which once again there is no clear glaring trend. From a more detailed look, a possible pattern could be extracted, by dividing the area into regions of power consumption. In the top one, roughly above 2.2 W, the configurations with long and medium queue lengths seem to be the predominant ones in all the Pareto fronts. In contrast, in the medium region, for powers between 1.8 W and 2.2 W, the longest queue seems to be replaced by the unitary one. For the bottom region, all configurations appear quite randomly, probably an indication that for such a rate, only rate 10 falls into that region, queue length does not play a significant role. 
\begin{figure}
    \centering
    \includegraphics[width=.85\columnwidth]{images/aoi/pareto_front_delay_fifo.pdf}
    \caption{Pareto fronts for FIFO delayed configurations}
    \label{fig:pareto_front_delay_fifo}
\end{figure}

The Pareto fronts are reported also for the head-drop configurations in \ref{fig:pareto_front_delay_drop}. From the analysis of the graph, the same consideration emerges, i.e. \acrshort{quic} dominates in terms of \acrshort{aoi}, but with greater power consumption. Moreover, the nature of the head-drop queuing policy obtains benefits also for high rates, but extracting other useful information from the curves is not an easy task, because the rate appears quite randomly on the fronts, especially for higher delay values. 
\begin{figure}
    \centering
    \includegraphics[width=.85\columnwidth]{images/aoi/pareto_front_delay_drop.pdf}
    \caption{Pareto fronts for Head-Drop delayed configurations}
    \label{fig:pareto_front_delay_drop}
\end{figure}
From the analysis of the Pareto fronts, some insights have been extracted despite at first glance it may seem a random placement of points. However, the study shows no significant variation in the optimal configuration as the delay and thus the operating scenario changes. 
Please note that from both Pareto fronts, some points were discarded because obtained with an inaccurate synchronization between \acrshort{rpi} and the laptop.

\subsubsection{Payload size}
The \acrshort{aoi} experiments reported so far were all conducted with a fixed payload of 128 bytes, which represents a reasonable size for an \acrshort{iot} scenario in which sensor readings are transmitted to a collection point. However, there may be scenarios where more advanced sensors are employed or data coming from multiple sensors attached to the same device are merged in the same message, potentially exceeding in both cases the amount of data fixed in the experiments. From this consideration, some experiments with a larger payload size have been carried out, to spot any meaningful difference in these new scenarios. In particular, were chosen payloads up to 2048 bytes, able to accommodate a quite large amount of data in a single application message. The choice of 2048 bytes allows also to account for any possible effect on the \acrshort{aoi} for application messages that cannot fit in a single segment of the transport layer. Regarding the transmission rate for the experiment only rates up to 1000 messages per second have been considered, mainly for two reasons:
\begin{itemize}
    \item From precedent experiments the best configurations resulted in the one with a real transmission rate of around 1000/2000 messages per second.
    \item Large payload size and high transmission rate would produce a very high throughput requirement, not sustainable by the \acrshort{rpi} and in general by an \acrshort{iot} device that may have even more constrained resources.
\end{itemize}
as a consequence, the choice was to limit the maximum rate to 1000 messages per second.

Starting again from the time evolution analysis \acrshort{aoi}, there is nothing special to report until the most resource-demanding configurations, i.e. 2KB payload and rate 1000, for all queuing policies and transport protocols. The time evolution assumes different shapes, according to queue size and transport protocol highlighting different behaviours of the configurations for this operating region. The first time evolution reported, \ref{fig:aoi_time_evolution_2KB_Q1024_R1000}, refers to the FIFO-1024 configuration. The trend for both transport protocols is clear, the system is not able to handle the throughput required by the configurations, and after an initial transitory phase, the \acrshort{aoi} assumes the usual shape, although rather irregularly, at a higher quote than the expected one. The explanation for this trend is given by the long application queue employed, which once fully forces the message generation to adapt to the transmission rate. So, after an initial transitory during which the queue is filled, the \acrshort{aoi} encounter a steady situation posing a limit to the divergence trend, but remaining at very high \acrshort{aoi} values, in the order of seconds. The same figure also highlights a difference between \acrshort{quic} and \acrshort{tls}, with the former showing, albeit in the same order of magnitude, a better \acrshort{aoi}, i.e. reach a steady state at a lower quote. Moreover, the \acrshort{quic} curve is characterised by a recurring trend, with an upward peak followed by a downward peak. 
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/aoi_time_evolution_2KB_Q1024_R1000.pdf}
    \caption{Time evolution for 2KB, FIFO 1024, Rate 1000}
    \label{fig:aoi_time_evolution_2KB_Q1024_R1000}
\end{figure}
The better behaviour of \acrshort{quic} in this scenario is confirmed by the FIFO-16 configuration, for which the initial transitory is quite reduced. In general, both transport protocols achieve benefits in terms \acrshort{aoi} by reducing the queue length because, once the steady state is reached, the \acrshort{aoi} is dominated by the number of messages preceding it in the queue, which will take time to be transmitted, ageing the last message entered.

The application queue seems to be the cause of the dramatic increase of the \acrshort{aoi}, so for FIFO-1 and even better for the head-drop configuration is legit to expect a significant improvement, but the time evolution plotted for the configuration, don't confirm this intuition. In \ref{fig:aoi_time_evolution_2KB_Q0_R1000} is reported the time evolution for the head-drop configuration, characterized by no application queue, in which is possible to observe that the median value for \acrshort{quic} is around 500 milliseconds and for \acrshort{tls} about 1300 milliseconds. These high values could be justified if the time required to fully transmit the message would be in that order of magnitude, but given the available bandwidth, \ref{tab:net_stats}, this is not a viable option. The high value for \acrshort{aoi} in the head-drop queue and the strange trend of \acrshort{quic} configurations, characterised by the recurring peaks that are hardly justified limiting the analysis to the application layer, suggest that an oversized buffering, that takes place somewhere between the transmitter and the receiver, might be the cause of the poor results. Such buffering is responsible for the queuing packets that can't be immediately transmitted without reducing the transmission rate from the application point of view. This results in a large amount of data being handled, delaying the delivery of the enqueued messages and thus the experienced latency and consequently the \acrshort{aoi}. If the buffering takes place inside the transmitter the phenomenon is indicated as on-device buffer-bloat and as studied in \cite{bufferbloat}, it may arise also for upload traffic, typically characterised by a slower data rate with respect to the download traffic. The source of buffering may be multiples and the final result could be a sum of all of them. 
\begin{itemize}
    \item \textbf{Kernel}, the TCP/IP stack implemented in the kernel involves several buffers, which may account for a non-negligible queue time. 
    \item \textbf{Cellular firmware}, inside the cellular network card there may be rather long queues that can't be directly controlled via software but are handled by the device's firmware itself. 
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/aoi_time_evolution_2KB_Q0_R1000.pdf}
    \caption{Time evolution for 2KB, Head-Drop, Rate 1000}
    \label{fig:aoi_time_evolution_2KB_Q0_R1000}
\end{figure}
Given the computational resources of the server in the University of Pisa cloud, hosting the \acrshort{mqtt} broker, it is safe to assume that buffering will not occur on the receiving side. However, the buffering may still occur outside the transmitter, in particular in the cellular network infrastructure, approximately in the vicinity of the base station, indicated as eNodeB in the \acrshort{lte} infrastructure. The latter hypothesis can be verified by a simple experiment involving measuring the \acrshort{rtt} toward intermediary hops via traceroute, or a similar command for idle network conditions and then for a loaded network, e.g. while running a speed test to saturate the network capacity. This simple test showed an increasing \acrshort{rtt} both during the download and upload phase of the data traffic, however, the increase considering a simple \acrshort{rtt} captured via \acrshort{icmp} packets explains only partially the abrupt increase in the \acrshort{aoi} experienced in the experiments. The results, reported in \ref{tab:mtr-echo}, show a slighter worse \acrshort{rtt} during the upload phase, which can be justified by a lower bandwidth. Moreover, in the first hop, which is the modem in the cellular network card connected to the \acrshort{rpi}, the \acrshort{rtt} stays on low values, so it allows to exclude the kernel buffers from the analysis. The second hop, which is the first IP component in the cellular infrastructure, is configured to not reply to ICMP packets. However, it is reasonable to state that the buffer should be located by the first two hops, the ones that typically act as bottlenecks. The buffer may also be present on both hops since the phenomenon is experienced in both directions.
\begin{table}
    \centering
    \caption{Traceroute output for loaded network}
    \label{tab:mtr-echo}
	\begin{tabular}{lrr}
		\toprule\toprule
		\multicolumn{1}{c}{\textbf{Hop}} & \multicolumn{1}{c}{\textbf{\acrshort{rtt} during download}} & \multicolumn{1}{c}{\textbf{\acrshort{rtt} during upload}}\\
		\midrule
		mobileap.qualcomm.com & 5.1 & 4.3 \\
        \midrule[0pt]
        - & - & - \\
		\midrule[0pt]
        192.168.10.30 & 413.2 & 528.4 \\
		\midrule[0pt]
	    192.168.255.5 & 444.3 & 540.8 \\
            \midrule[0pt]
		ppp64-paris2.isdnet.net & 606.8 & 558.3 \\
            \midrule[0pt]
		194.149.189.44 & 423.0 & 421.1 \\     
            \midrule[0pt]
		194.149.186.32 & 379.1 & 640.8 \\      
            \midrule[0pt]
		garr.mix-it.net & 616.6 & 666.1 \\        
            \midrule[0pt]
		re1-mi02-rs1-rm02.rm02.garr.net & 672.5 & 744.5 \\       
            \midrule[0pt]
		rx1-pi1-ru-unipi.pi1.garr.net & 766.5 & 765.2 \\           
            \midrule[0pt]
		jser-jspg.unipi.it & 669.3 & 721.2 \\         
            \midrule[0pt]
		broker.mqtt.unipi & 581.9 & 655.8 \\
        \bottomrule
	\end{tabular}
\end{table}

Moving on to the comparison between transport protocols it is interesting to note that although \acrshort{tls} is still the least power demanding, while \acrshort{quic} provides a better \acrshort{aoi}, by increasing the payload size the energy difference between the protocols tends to shrink, especially for the FIFO queuing policy. In \ref{fig:power-comparison-q1} is reported this trend for the configuration FIFO-1. The trend is partially reflected also in the \acrshort{aoi}, so the Pareto front obtained for these configurations is pretty similar to the one analysed so far. From the graph, although it is not so obvious, it can be seen that, as expected, energy consumption increases as the payload size gets larger. 
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/payload_power_comparison_Q1.pdf}
    \caption{Power comparison varying the payload size for FIFO-1}
    \label{fig:power-comparison-q1}
\end{figure}

From the latter graph, although it is not so glaring, it can be seen that, as expected, energy consumption increases as payload size gets larger. Still, regarding the \acrshort{aoi} a counter-intuitive result is obtained, in fact, the median \acrshort{aoi},  basically for all configurations, decreases as the payload increases for the rate 100 and some configurations even 1000, except for the 2 kilobytes payload. \ref{tab:aoi-payload-tls-q16} shows this peculiar trend, for which a deeper analysis is required to understand the underlying phenomenon responsible for this decrease.

\begin{table}
    \centering
    \caption{Median \acrshort{aoi} varying the payload size for \acrshort{tls}, FIFO-16, rate 100 configuration}
    \label{tab:aoi-payload-tls-q16}
	\begin{tabular}{lr}
		\toprule\toprule
		\multicolumn{1}{c}{\textbf{Payload size}} & \multicolumn{1}{c}{\textbf{Median \acrshort{aoi}}} \\
		\midrule
		128B & 107.38 \\
		\midrule[0pt]
        256B & 85.04  \\
		\midrule[0pt]
		512B & 65.52  \\
        \midrule[0pt]
		1KB & 60.24  \\
        \midrule[0pt]
		2KB & 55.46  \\
		\bottomrule
	\end{tabular}
\end{table}

For completeness, the Pareto front for 2 kilobytes payload is reported in \ref{fig:pareto-front-2kb}. The selected front is the only one that shows some differences from the other, having the best configurations in terms of \acrshort{aoi} for the rate of 100 messages per second due to the problems caused by the intense upload traffic generated at higher rates. The same can be shown also for the head-drop Pareto front, reported in \ref{fig:pareto-front-2kb-drop}.

\begin{figure}
    \centering
    \includegraphics[width=.85\columnwidth]{images/aoi/pareto_front_P2KB.pdf}
    \caption{Pareto front for FIFO 2KB payload configurations}
    \label{fig:pareto-front-2kb}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.85\columnwidth]{images/aoi/pareto_drop_P2KB.pdf}
    \caption{Pareto front for Head-Drop 2KB payload configurations}
    \label{fig:pareto-front-2kb-drop}
\end{figure}

\subsubsection{Multiple cores}
The developed software tool runs employing only one thread, implementing concurrency through asynchronous mechanisms. Those mechanisms should maximise the usage of computational resources, exploiting the idle times dictated by waiting for I/O operations to carry out other tasks. The advantage respected to standard multi-threaded implementation is a lightweight switching from one task to another, keeping also in mind that only one core is enabled in the \acrshort{rpi}. Having only one core doesn't allow for true concurrency. i.e. only one thread can be executed at a time. This should not be a problem since the developed tool is a single-threaded software, however, it must be taken into consideration that the application has a tight interaction with the kernel that is responsible for completing the network operations. The details of kernel implementations are out of scope for this thesis, but typically more kernel threads could be involved, competing with the application one for the computational resources. From this consideration may be interesting to observe what happens enabling another core in the system, thus allowing for a true parallelization of the operations. For this experiment, all the rates have been considered because is interesting to spot if greater computational power allows for higher transmission rates for the configurations without a large space in the queue.\\
The time evolution graphs do not highlight any difference from the base ones, so they are not reported. The analysis of maximum reachable rates confirms the hypothesis of benefits from the second core, showing a higher transmission rate for the FIFO configurations, in particular, the improvement is evident for FIFO-1. In \ref{fig:aoi_cores_comparison}, it is possible to observe such improvement for the \acrshort{quic} configuration, indicated by the orange line, representing the 2-cores version, extending more than the blue one. Moreover, quite interesting, can be noted that the effect of the second core isn't limited to reaching a higher rate, but more importantly, has a positive impact on the \acrshort{aoi}. Note that in the figure the slowest rate has been cut off to avoid excessive enlarging of the y-scale and also the points having nominal rate not reachable are not present in the graph. Regarding the head-drop queuing policy, the addition of the second core does not seem to cause any effect, producing results quite similar to those obtained with only one core enabled. This result could be justified by the overwrite possibility of the queuing policy, which limits the required computational power, easily handled even with only one enabled core. This hypothesis should be better investigated, for example by monitoring the per-core utilization during the configuration running.
\begin{figure}
    \centering
    \includegraphics[width=.85\columnwidth]{images/aoi/aoi_cores_comparison.pdf}
    \caption{\acrshort{aoi} comparison enabling second core for \acrshort{quic}, FIFO-1}
    \label{fig:aoi_cores_comparison}
\end{figure}
The positive impact of the second core has a drawback, paid in terms of additional energy required to power the hardware component. This consequence is quite obvious, however, observing the comparison between the power needed by the device in both configurations some unexpected results spot out. 
\begin{itemize}
    \item \textbf{Head-drop queue}, energy results mirror those of rates and \acrshort{aoi}, returning very similar energy consumption results despite the addition of the second core.
    \item \textbf{FIFO queue}, the impact on the energy consumption is significant only for high rates, associated with higher computational loads. The difference is greater for configurations whose second core allows for a higher transmission rate, and this is explained by the fact that in addition to the extra energy required by the core, the higher rates increases also the power consumption of the network card.
\end{itemize}
In \ref{fig:energy_cores_comparison} the just described trend is reported. In the left figure, \acrshort{quic} and head-drop configuration, it can be seen that the bars are very close regardless of the rate considered, with the differences due to statistical variations. In the figure on the right, \acrshort{quic} and FIFO-1 configuration, starting from the speed of 3000 messages per second, instead a significant difference can be appreciated between the single-core and the dual-core version.
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/aoi_cores_energy_comparison.pdf}
    \caption{Energy comparison enabling second core for \acrshort{quic}, FIFO-1 and Head-Drop}
    \label{fig:energy_cores_comparison}
\end{figure}

Finally, the Pareto front doesn't appear so interesting since the only consideration that can be applied resembles the one already pointed out for the other experiments. The only observation that can be made concerns the absence of FIFO-16 configurations as optimal points, but the proximity of these points to the front excludes the possibility that this is a phenomenon given by the scenario under analysis. The same applies also to the head-drop Pareto front.

\subsubsection{Final experiments}
The experiments presented so far have shown many aspects of the \acrshort{aoi} and energy combined study. However, it is worth pointing out some limitations in the study, in particular regarding the lack of repetition not consent to properly filter out the noise from the collected data and thus sometimes not to draw accurate conclusions. Moreover, the parameter choice can be improved to collect more data in more interesting regions. For example, the rates above 2000 messages per second are not so interesting due to the saturation of resources and the same applies to the rate 1. A final experiment is presented below to overcome these limitations, for which 30 repetitions were performed. The parameters adopted for this experiment are listed in the \ref{tab:aoi_parameter_space_final}. The \acrshort{tls} version with Nagle's algorithm disabled is added in the configurations since as analysed the aggregation at the transport level plays a crucial role for the \acrshort{aoi} and the maximum reachable rate, often resulting in the discriminant factor between \acrshort{quic} and \acrshort{tls}. The queuing policies have been streamlined, maintaining just one version per type, i.e. the head-drop approach and a single FIFO length, specifically FIFO-16. This decision is to prioritize the comparison of transport protocols, which has now expanded from two to three options. Regarding the transmission rates, they are chosen in such a way as to obtain a dense collection of measurements up to the upper limit of 2000 messages per second. The pattern followed to set rates is 5-10-20, multiplying by 10 each cycle until 2000 is reached, for a total of 9 transmission rates. Finally, the other parameters inherit the base configuration, the first analysed in this experiment campaign. The experiment comprises a total of 54 configurations, each executed 30 times, resulting in a total of 1620 runs. With each run taking approximately 80 seconds to complete, the entire set of experiments required approximately 36 hours to finish.
\begin{table}
	\centering
	\caption{\acrshort{aoi} final experiment parameter space}
	\begin{tabular}{lcl}
		\toprule\toprule
		\multicolumn{1}{c}{\textbf{Parameter}} & \multicolumn{1}{c}{\textbf{Unit of Measure}} & \multicolumn{1}{c}{\textbf{Value}} \\
		\midrule
		Transport protocol & - & \acrshort{tls}, \acrshort{tls} (Nagle Disabled), \acrshort{quic} \\
		\midrule[0pt]
        Payload size & [B] & 128\\
		\midrule[0pt]
		Delay & [ms] & 0 \\
        \midrule[0pt]
		Bandwidth & [Mbit/s] & 100\%\footnotemark \\
        \midrule[0pt]
        Access network& - & 4G \\
        \midrule[0pt]
        Time window & [s] & 60\\
        \midrule[0pt]
        Queue policy & - &FIFO-16, HEAD-DROP\\
        \midrule[0pt]
        Generation rate & [msg/s] & 5, 10, 20, 50, 100, 200, 500, 1000, 2000 \\
        \midrule[0pt]
        CPU cores & - & 1 \\
		\bottomrule
	\end{tabular}
	\label{tab:aoi_parameter_space_final}
\end{table}
\footnotetext{No bandwidth restriction}
The analysis of the collected data required an aggregation of the repetitions, each producing the usual metrics reported so far, i.e. mean and median value for the \acrshort{aoi} and the power consumption of the configuration. The aggregation employs the median value of the set of metrics, which can be easily applied since the set is composed of scalar quantities.
\bigbreak
The results for both queuing policies have rather similar trends. This similarity comes from the fact that the largest differences are obtained from higher rates, which were not considered in this final experiment. However, some differences are still appreciable and will be highlighted in the following.

The first result reported, \ref{fig:aoi-fifo-repetition}, is the \acrshort{aoi} obtained varying the transmission rate for the FIFO-16 configurations. From the graph, it is possible to observe some interesting facts about the comparison between transport protocols and the trend of standard \acrshort{tls}. First of all, the \acrshort{quic} better behaviour in terms of \acrshort{aoi} with respect to the standard \acrshort{tls} is confirmed also by the repetitions, but the most important result is that disabling Nagle's algorithm \acrshort{tls} yields the same if not slightly better, results as \acrshort{quic}. This result shows that the main difference in terms of \acrshort{aoi} between the transport protocols is given by the aggregation mechanism at the transport layer, much more aggressive when Nagle's algorithm is enabled. 

The other observation valid for the reported graph is about the strange trend of \acrshort{tls} for rates between 10 and 100 messages per second. The \acrshort{aoi} decreases as expected passing from rate 5 to rate 10, but then further increasing the rate to 20 messages per second produces a negative effect that will vanish only after approaching rate 100, for which the \acrshort{aoi} is roughly equivalent to the local minimum of rate 10. In the case of a single measurement such behaviour would be treated as noise, but the curve is obtained aggregating 30 repetitions, so the noise can't be the cause. The fact that this trend stands out only for the standard \acrshort{tls} suggests that the phenomenon is triggered once again by Nagle's algorithm. Moreover, so far this trend has been hidden by the absence of points in the region of interest, recalling that previous experiments only provided rates of 10 and 100 and not intermediate ones. The explanation is obtained by observing that the rates under analysis are those having a transmission period similar to the \acrshort{rtt} of between \acrshort{rpi} and the broker. First of all, it's worth recalling that the communication is bidirectional, i.e. the producer sends messages to the broker which in turn replies with application acknowledgements. Those reply messages are enveloped into a \acrshort{tcp} segment that is sent towards the publisher, transporting at the same time also the acknowledgement at the transport layer, which assumes an important role in Nagle's algorithm, allowing to flush pending messages that have not yet saturated a segment. The \ref{fig:tls-nagle-effect} reports a simple scheme which allows better visualization of the communication pattern. When the transmission period is greater than the \acrshort{rtt}, the bidirectional exchange completes before the generation of the new message, Nagle's algorithm doesn't get involved because each time data arrives from the application level there aren't pending acknowledgements, so the segment can be sent immediately out. For those configurations, the \acrshort{aoi} is completely determined by the rate established. When the transmission period becomes shorter then the \acrshort{rtt} Nagle's algorithm comes into play because new messages are generated before the reception of the broker's reply and thus the pending acknowledgement of the transport layer. In such a scenario, the algorithm delays the segment transmission until the reception of the acknowledgement or the segment gets full. The experienced delay and the aggregation level depend on how messages are combined and by the exact \acrshort{rtt} for each exchange. In any case, the \acrshort{aoi} is negatively affected by this aggregation, resulting in a worse median value despite the increase of the transmission rate in a not-overloaded condition.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/aoi_fifo_repetition.pdf}
    \caption{Median \acrshort{aoi} over transmission rate for FIFO-16 configurations}
    \label{fig:aoi-fifo-repetition}
\end{figure}

\begin{figure}
    \begin{minipage}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/aoi/nagle_effect_1.pdf}
        \subcaption{Transmission period larger than RTT}
    \end{minipage}
    \begin{minipage}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/aoi/nagle_effect_2.pdf}
        \subcaption{Transmission period smaller than RTT}
    \end{minipage}
    \caption{Effect of Nagle's algorithm on the \acrshort{aoi}}
    \label{fig:tls-nagle-effect}
\end{figure}

The \acrshort{aoi} improvement obtained by removing the aggregation has a consequence from the energy point of view, as shown in \ref{fig:power-fifo-repetition}. The \acrshort{tls} curve with Nagle's algorithm disabled is much closer to the \acrshort{quic} curve instead of the standard \acrshort{tls} curve. However, the \acrshort{quic} configuration seems to be the most energy-demanding, at least up to the highest considered rate, for which the curves swap. The lack of aggregation in the \acrshort{tls} with Nagle's algorithm disabled may be the cause of the inversion. The \acrshort{quic} protocol is responsible for lighter aggregation than Nagle's algorithm, so the effects on the \acrshort{aoi} are limited, but when the transmission rate increases having some messages shipped in the same transport layer packet allows for fewer transmissions and therefore less energy spent. A simple analysis of traces collected for a rate of 2000 packets per second shows a mild aggregation for \acrshort{quic}, around 2 messages per segment, while \acrshort{tls} without Nagle's algorithm doesn't provide any form of aggregation.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/power_fifo_repetition.pdf}
    \caption{Power over transmission rate for FIFO-16 configurations}
    \label{fig:power-fifo-repetition}
\end{figure}

\bigbreak
It's worth recalling that despite the 30 repetitions, when the curves are very close, for both figures, is not possible to state that a configuration is better than the other. To furnish a precise result some statistical methods should be applied, such as the confidence interval. The statistical methods work well under certain circumstances, that are not always easy to meet or prove, so an inaccurate usage may give a false confidence ending up in a not optimal decision.
However, in the Pareto front apart from the median value the $25^{th}$ and $75^{th}$ percentiles for both \acrshort{aoi} and power will also be reported for more detailed comparison without getting involved in too rigorous methods. The Pareto front reported in \ref{fig:pareto-fifo-repetitions}, was constructed differently from those analyzed so far, in particular, the fronts for each transport protocol considered are first drawn, jointly with an upper and lower bound both horizontally and vertically, given by the percentiles mentioned above. Then the final Pareto front is obtained merging the best front in each region. The introduction of percentiles transforms a simple curve into a band with a vertical and horizontal extension. A larger band means a greater variability of data and thus less confidence in the single point obtained via aggregation. When the bands are far enough is quite safe to state that one solution is better than the other, however, if the bands intersect each other, the two solutions are almost equivalent and thus the choice should be taken considering other aspects. Back to the reported Pareto front, the bands tend to intersect multiple times, however, it is possible to make some conclusions. In the right part of the graph, the transport protocols behave similarly and such similarity could be better highlighted if the x-axis wouldn't be cut for values greater than 100. Moving towards the left, the \acrshort{tls} dominates the other protocols, leaving a space from one band to the others and having the Pareto front completely in its band. Keeping moving in the same direction the standard \acrshort{tls} is not able to guarantee the optimal results, so it is replaced by the other two protocols, for which there isn't a clear winner.
\begin{figure}
    \centering
    \includegraphics[width=0.85\columnwidth]{images/aoi/pareto_front_repetition_fifo.pdf}
    \caption{Pareto fronts for FIFO configurations}
    \label{fig:pareto-fifo-repetitions}
\end{figure}

Regarding repetitions for head-drop configurations, as already anticipated, the trend in \acrshort{aoi} and power are identical to the FIFO case, except that the maximum achievable rate is less than 2000 for all the transport protocols. The \acrshort{aoi} and power trend over the rate are reported for completeness in \ref{fig:aoi-drop-repetition} and \ref{fig:power-drop-repetition}.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/aoi_drop_repetition.pdf}
    \caption{Median \acrshort{aoi} over transmission rate for Head-Drop configurations}
    \label{fig:aoi-drop-repetition}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/aoi/power_drop_repetition.pdf}
    \caption{Power over transmission rate for Head-Drop configurations}
    \label{fig:power-drop-repetition}
\end{figure}

The Pareto front, \ref{fig:pareto-drop-repetitions}, for the head-drop configuration, is built in the same manner as the previous one. Also for this Pareto front for most of the graph, the bands intersect each other, however after the initial equivalence of the protocols, the \acrshort{tls} with Nagle's algorithm disabled dominates the other for a short interval and then the standard \acrshort{tls}, mirroring the results of FIFO configurations, results in the best even if the bands are not completely separated. In the highest part of the graph, \acrshort{quic} and \acrshort{tls} with Nagle's algorithm disabled dominates obtain better results, but being very close no further conclusion can be derived.

\begin{figure}
    \centering
    \includegraphics[width=0.85\columnwidth]{images/aoi/pareto_front_repetition_drop.pdf}
    \caption{Pareto fronts for Head-Drop configurations}
    \label{fig:pareto-drop-repetitions}
\end{figure}

An interesting aspect of the Pareto fronts is that \acrshort{quic} presents a larger variability, indicated by a larger band, especially for slower rates, i.e. on the right part of the graphs, while both versions of \acrshort{tls} generate a narrower band. Moreover, the Pareto fronts show that the aggregation of Nagle's algorithm can save energy, paying a higher \acrshort{aoi}. The result is that for a middle region, where the \acrshort{aoi} is not minimized, the standard \acrshort{tls} seems to guarantee the best trade-off. When the requirements on \acrshort{aoi} are the most stringent then the aggregation limits the performance, thus disabling Nagle's algorithm or adopting \acrshort{quic} as transport protocol could help to meet the requirements.

The overall comparison between \acrshort{quic} and the two versions of \acrshort{tls} doesn't determine a clear winner able to provide the best results in any scenario. However, there are many differences, and some features may steer the choice toward a certain configuration rather than another. The simple fine-tuning of the \acrshort{tls} protocol, derived from the underlying \acrshort{tcp} option, can guarantee optimal protocol results even in those scenarios where \acrshort{quic} seemed to guarantee better results, so in many cases the greater availability of \acrshort{tls} may favour this protocol over the emerging \acrshort{quic}, for which the standardization process and availability are not yet comparable to the classic \acrshort{tls} over \acrshort{tcp}.

==> thesis-sections/background.tex <==
\section{Background}
\label{sec:related-works}
\subsection{Quic in the Internet of Things}

The \acrshort{iot} domain is currently one of the hottest topics in the research field, characterized by a vast body of published studies contributing to an extensive literature. Among the various published works,  there is a growing number of studies about the recent \acrshort{quic} transport protocol and its applicability in a resource-constrained environment. In \cite{Eggert2020TowardsST} the authors tested the feasibility of a \acrshort{quic} standard implementation designed for tiny devices. Specifically, they quantified the storage, computing, memory and energy requirements of the Quant \acrshort{quic} \cite{NTAP_quant} implementation on different \acrshort{iot} platforms. The implementation they tested showed a binary footprint of less than 100KB without any optimisation during the compilation process and a reduction in size to 58KB by adding some optimisations at the compilation stage and removing some components that may not be required. Regarding memory utilization, they monitored the memory occupied during a 5KB download transfer from a local server. The results showed a moderate stack allocation size during the transfer and closing phases of the connection, around 1KB, while in the connection establishment, the stack allocation reached peaks over 3KB, mainly due to the asymmetric cryptography involved in the initial key-exchange phase of \acrshort{tls}. The analysis on heap memory showed a rather stable behaviour during the execution phase, mainly due to the preallocation of structures in the init phase of the \acrshort{quic} implementation. Finally, in terms of energy, they repeated in a loop the download from the server, consuming less than one joule per connection. The study revealed the feasibility of the \acrshort{quic} protocol, but it was limited to raw data transfer, without involving any application protocol. The studies regarding \acrshort{quic} as a transport layer below an application protocol are mainly focused on \acrshort{http} since the new transport layer was introduced to replace \acrshort{tcp} within the Chromium project. Some of the studies on \acrshort{http} and \acrshort{quic} are framed in the \acrshort{iot} domain, such as \cite{http-quic-iot}. The authors carried out a study in an \acrshort{iot} cloud/edge continuum scenario, a solution that is gaining popularity based on the integration between \acrshort{iot} and cloud/edge systems. They realized a setup composed of variable numbers of emulated \acrshort{iot} nodes sending data to an \acrshort{http} server hosted on an edge node, which in turn sends data to the cloud for storing purposes. The communication leveraged the application protocol \acrshort{http}/3, the \acrshort{quic} based version. They tested the latency and scalability experienced in the system, in particular, they measured the \acrshort{rtt} required by a \acrshort{http} message exchange from an \acrshort{iot} node to the edge node or the cloud. The tests were carried out varying both payload size, from 10B to 1KB, and the number of emulated devices, from 1 to 500. The results showed that latency and scalability are an open challenge for \acrshort{http}/3, obtaining results in the order of hundreds of milliseconds for the latency in an unloaded scenario and in the order of seconds increasing the number of \acrshort{iot} devices in the system.
Recently the \acrshort{quic} protocol gained attention also as the underlying transport layer for popular application protocols in the \acrshort{iot} domain, such as \acrshort{mqtt} specifically designed to implement a lightweight publisher-subscriber message exchange pattern.
In \cite{iot-meets-quic} Fatima et al. recognise the limitations of \acrshort{tcp} in an industrial \acrshort{iot} context, characterised by lossy networks and at the same time by stringent latency requirements. To cope with this problem, they assessed the potential of \acrshort{quic} as a transport layer below the application protocol \acrshort{mqtt}. They built an ad-hoc configuration, using a network simulator capable of reproducing different wireless technologies, varying latency and available bandwidth. They compared the time required for the completion of a series of \acrshort{mqtt} message exchanges above \acrshort{tcp}/\acrshort{tls} and \acrshort{quic}. They analysed two scenarios, in the first the same connection is used to send a predetermined number of published messages to the broker that in turn forward them to the subscriber. In this scenario they found out that \acrshort{quic} outperforms \acrshort{tcp}, obtaining even a larger improvement when introducing a frame error rate, up to a 40\% faster completion. The behaviour is the same for all the simulated networks, even if the ones characterised by a larger \acrshort{rtt} show a smaller difference between the two transport protocols. In the second scenario, the authors examined the performance of both protocols involving short-lived connections, where the connection is terminated immediately after message publishing. They aimed to highlight the advantages of \acrshort{quic}'s lightweight connection establishment. Surprisingly, the results demonstrated comparable performance between the two protocols. The authors identified a misconfiguration in the \acrshort{quic} protocol as the cause of this unexpected outcome and planned to address it in future studies. Their work, in particular the simulation environment, poses the base for the study conducted in \cite{quic-iot-gateway}, where the benefits of \acrshort{quic} as transport layer are analysed again for a \acrshort{iot}-cloud interaction. They compared the time needed for a \acrshort{mqtt} session composed of connection establishment and message publishing taking into account \acrshort{quic} and \acrshort{tcp}/\acrshort{tls} transport layers. They observed a supremacy of \acrshort{quic} protocol, further improved by enabling 0-\acrshort{rtt} mechanism, as it was capable of reusing cryptography material from past sessions to avoid a new \acrshort{tls} handshaking. They analysed also the case in which the broker hosted in the cloud doesn't support \acrshort{quic} protocol, installing a local gateway able to perform a conversion of transport protocol toward standard \acrshort{tcp}/\acrshort{tls} connection. In this scenario the time required by the \acrshort{iot} device, compared with a direct \acrshort{tcp}/\acrshort{tls} connection toward the broker, still improved employing \acrshort{quic}, even if the time recorded on the broker expanded since the conversion on the gateway requires time.\\
Fatima et al. extended their work, presented above, in \cite{energy-quic-mqtt} setting up a real test-bed to profile \acrshort{quic} both in terms of energy and delay, two key indicators in the \acrshort{iot} field. Their setup mimics an \acrshort{iot} system communicating via wireless technology to a broker hosted in the cloud, jointly to the subscribers represented by services requiring data collected in by \acrshort{iot} nodes. Their setup lacks a truly wireless connection, simulated imposing some restriction to an Ethernet connection between the \acrshort{iot} device and the one acting as a virtual machine hosting the broker in the cloud. The choice was justified by the greater control over the connection, allowing for fair conditions in the measurements of different configurations. The first results they show are related to the delay experienced by \acrshort{mqtt} messages, obtaining lower delay and better stability results for \acrshort{quic} especially introducing an error rate in the connection link. They also analysed the behaviour of delay varying the \acrshort{qos}, observing that for low latency networks, the difference is limited, while increasing the latency higher \acrshort{qos} accounts for a much higher experienced delay. Finally, they measured the energy required for their experiments made up of 1000 \acrshort{mqtt} message publishing obtaining firstly comparable results employing an ideal connection, i.e. without losses or limitations. Then they tried to enlarge the study on the simulated wireless technologies but some limitations on their instruments imposed only an estimation of the power, based on the number of physical packets transmitted, observing a better behaviour of \acrshort{quic} for small or medium delays and contrary a slighter better result for \acrshort{tcp}/\acrshort{tls} in case of large delay.

\subsection{Age of Information}
The \acrshort{aoi} is a network-related metric employed to assess the freshness of data available to a collection point introduced somewhat recently in \cite{Kaul2011:minimizing}. The original work is framed in the vehicular network context, for which many nodes may transmit data in the single broadcast domain, resulting in a performance worsening due to packet collisions. They point out that the typical analysis at \acrshort{mac} layer is not sufficient for a system where the status information at each node plays an important role. Their work considers a more complex single aggregated value for the entire system, named system information age, obtained taking into account the end-to-end delay for all nodes in the network. The authors define $\Delta t_{uv}$ as the \acrshort{aoi} of node $u$ at node $v$ at time $t$. They also state that a node always has its current information, thus $\Delta t_{uu} = 0$. For nodes ${v \neq u}$, the state information of $u$ ages during the time between any two receptions from $u$. Also, the \acrshort{aoi} of any received information is the time that elapses between its generation and successful reception. Following the description provided by the authors the evolution in time of the \acrshort{aoi} assumes a sawtooth shape, increasing linearly between two message receptions and falling suddenly at the reception of a new message. Once defined the metric, they presented some implications in IEEE 802.11 networks, characterised by the \acrshort{csma} back-off mechanism for the medium access and queues needed to store outgoing packets managed by \acrshort{fifo} policy. In particular, starting from the observation that the time spent in the queue can increase when the throughput exceeds a certain rate, they first stated that the minimum \acrshort{aoi}, for the entire system, is obtained for an optimal operating point where the throughput is high and time spent in the queue is low. Then, adopting a simulation approach, based on queuing theory, they found out that a \acrshort{lifo} queuing policy has the effect of eliminating the queuing delay, even if setting short \acrshort{fifo} queues allows for a similar result. Moreover, they found out that contrary to \acrshort{fifo}, for \acrshort{lifo} policy maximizing the throughput allows reaching the minimum \acrshort{aoi} since it can be interpreted as sending as fast as possible the freshest information available. Their study acknowledges the fact that real systems work accordingly to a \acrshort{fifo} queue, requiring a different approach based on the choice of the optimal broadcast period, employing a distributed algorithm in the system.\\
The \acrshort{aoi} has gained more and more attention, evidenced by the thriving literature that can be found. However, most of it provides a theoretical study, mainly based on queuing theory or simulation-based approach. These studies suffer from modelling assumptions that may not reflected in the real case, thus providing results different to the one experienced in a real scenario. In \cite{Sonmez2018:age} the authors present one of the first experimental works on the \acrshort{aoi}. They aimed to validate the theoretical results of the non-monotonic convex relationship between \acrshort{aoi} and transmitting rate, i.e. a "U" shape of the \acrshort{aoi} over the transmitting rate. They first obtained a confirmation adopting an emulated approach, then they realized a real-world testbed composed of a cellular phone acting as a client and a remote server, synchronized each other for a correct \acrshort{aoi} computation. The experimental setup involved various network technologies and relied on the \acrshort{tcp} transport protocol. Overall they also validate the theoretical results employing an experimental approach, observing the expected shape for all the network technologies, differentiated mainly only by the point at which the \acrshort{aoi} starts to increase after reaching the minimum value. In \cite{Beytur2020:towards}, the authors conducted a study about \acrshort{aoi} for \acrshort{tcp} and \acrshort{udp} connections in a real environment. They used two test setups, the first involving three desktop PCs connected via the Internet and the second resource-constrained \acrshort{iot} devices communicating locally through WiFi. For the first setup the \acrshort{aoi} over the transmission they obtained the well-known "U" shape, for both transport protocols. The study highlighted some differences between \acrshort{tcp} and \acrshort{udp}, with the latter able to reduce the time spent in the queue since the protocol doesn't account for retransmission in case of packet loss, limiting the delay also for high rates. Regarding the \acrshort{iot} scenario they observed a different behaviour, given by the lack of resources on the devices able to saturate the communication module.\\
The \acrshort{fifo} queuing policy and \acrshort{csma} mechanism adopted by some network technologies appear to be the limiting factors for the \acrshort{aoi}. Some studies focused on implementing a mechanism able to solve both limitations without requiring a major refactor of the systems, such as \cite{Kadota2021:wifresh} in which the authors present their contributions to \acrshort{aoi} optimization, namely the WiFresh network architecture. They realized two implementations: one at \acrshort{mac} level, able to guarantee the best performance and one at the application level to reduce the complexity related to the modification of low network stack level. They showed promising results, scaling with the network size while keeping the \acrshort{aoi} at the lowest possible value. They reached those results by employing a polling multiple access mechanism to prevent packet collision, overcoming the problems due to the \acrshort{csma} access. The polling mechanism is based on a master node that in a centralized manner schedules the transmission of the other nodes in the networks, thus forcing the coordination. To maximize the benefits of the polling mechanism they also implemented a max-weight scheduling policy, that determines the optimal order of node transmission to minimize the overall \acrshort{aoi} in the system. Finally, they also introduced the \acrshort{lifo} queuing policy according to theoretical results showing such policy as the optimal one for \acrshort{aoi} minimization. The work presented in \cite{Chiariotti2021:quic} leverages some features of new transport protocol \acrshort{quic} to minimize \acrshort{aoi}
without requiring the definition of complex architectures. The authors focused on the multi-stream feature of the transport protocol, which allows treating each stream as a separate data flow with in-order reliable delivery, independent of other streams. The authors, taking a network of sensors as a reference, proposed to send each sensor's reading on a dedicated stream, extracting the first available from a pool to reduce the stream opening overhead. Their work took into account also the fact that the available network capacity may not be sufficient for all sensor readings, so they provided a scheduling mechanism to choose which data to transmit to maximize the value of the information, a metric related to the utility of the data, at the receiver. 

\subsection{Motivation}
The analysis of the previous works reveals considerable attention to topics related to the \acrshort{iot}, highlighting extensive coverage of these issues. In particular, the emerging protocol as \acrshort{quic} is gaining popularity as a modern alternative to the de-facto standard \acrshort{tcp} that showed limitations for lossy networks and constrained devices. The focus is also placed on the \acrshort{aoi} metric, able to represent the freshness of data that in modern systems assumes a pivotal role. However, some significant gaps emerged, in particular, the lack of experimental works, especially regarding the \acrshort{aoi} which could validate the large amount of theoretical results available in the literature. Also noteworthy is the void in the field of combined study on \acrshort{aoi} and energy, an area particularly interesting for the \acrshort{iot} context. This thesis is placed at the intersection of studies exploring energy consumption and \acrshort{aoi} in IoT, adopting an experimental methodology.

==> thesis-sections/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusion}

\subsection{Results}
The work presented aims to fill the gap in the literature about a combined study of energy consumption and \acrshort{aoi}, two metrics that play an important role in the \acrshort{iot} domain, especially for monitoring and controlling systems. Experimental results show that improving the AoI requires to increase the energy expenditure. This was somehow expected, as both metrics depend on the transmission rate, but the experimental results provide system designers with guidelines and numbers useful for finding the desired trade-off between AoI and energy consumption. The study revealed that the considered transport protocols have slightly different behaviors. Similarly, also the interplay between the transport protocol and the application level has an impact on the considered metrics. 

%The extensive experiment campaign validated the increasing interest in the \acrshort{quic} protocol for the \acrshort{iot} context. While from a performance point of view, there were already several studies admitting use in this context, the doubt regarding the energy implications of the protocol had not yet been addressed. 

The first experiment campaign highlighted an energy consumption for a single \acrshort{mqtt} publish message employing \acrshort{quic} as transport protocol not larger than the more widespread \acrshort{tls} on top of \acrshort{tcp}. In particular, the differences between the two transport protocols appear to broaden by introducing artificial delays in the network, with \acrshort{quic} showing also more stable results. 

The second experiment campaign is the real core of the work, in which the \acrshort{aoi} metric is extensively studied without losing attention to the energy, providing some insights for a missing piece in literature. The choice to develop a custom software tool to carry out the experiments allowed for maximum flexibility of the parameters to analyse. Aside from the comparison between \acrshort{quic} and \acrshort{tls}, the impact of the application queue policy and lengths has also been analysed, showing interesting results despite the lack of control on the lower part of the network stack. 

The use of Pareto fronts proved to be a useful conceptual tool to find the desired trade-off between \acrshort{aoi} and energy. Pareto fronts clearly highlight all the optimal solutions, leaving to the final designer the possibility to choose the operational point that better satisfies the specific system requirements. The results also showed better behaviour of the head-drop policy for the application queue management, but paying the cost of message loss which may not be admitted in some scenarios. For this reason, the analysis on \acrshort{fifo} is equally interesting, despite is not the optimal policy for the metrics under consideration. In particular, varying the queue length the system experienced a different efficiency in resource exploitation, maximized by employing long queues. 

Better resource exploitation is particularly relevant for the network since long queues allow for aggregation at the transport level resulting in a dramatic improvement in terms of reachable throughput. The aggregation at the transport layer was revealed to be a paramount factor to take into consideration, explaining many differences between configurations and odds behaviour observed during the presentation of the results. The aggressive aggregation enforced by Nagle's algorithm, a standard mechanism enabled for \acrshort{tcp} connections, is the main factor causing different results for the two transport protocols, with \acrshort{quic} able to guarantee a better \acrshort{aoi} at the cost of higher energy consumption, at least for the rates employs in the analysis. This difference disappears disabling Nagle's algorithm, improving the \acrshort{aoi} performance of \acrshort{tls}, but at the same time requiring more energy due to the more frequent transmission. 

Overall, the study confirmed the possibility of adopting \acrshort{quic} as a reliable transport protocol, replacing \acrshort{tcp}, however, the immaturity of the new protocol may represent an obstacle to its adoption, favouring a more standardized protocol for which compatibility and support are much larger.  

\subsection{Limitations and future work}
The experiments conducted for the study limited the analysis to the top levels of the network stacks, namely application and transport, without taking into account lower-level details. The choice is justified by the willingness to operate at a level for which the adopted techniques can be reproduced also in a real context where the development time is often one of the tightest requirements to meet. Operating at a lower level may also limit the study to a specific target, thereby losing generality. However, the interplay of lower levels may highlight some aspects left in shadow in the presentation of the results, finding an explanation for some of the open questions. Moreover, the effects of external factors out of control should be better isolated, such as the bufferbloat phenomenon experienced for loaded network conditions.
The features of \acrshort{quic} protocol may be better exploited for future studies, employing the multi-streaming mechanism to bypass at the transport layer the strict \acrshort{fifo} queuing policy by using a single connection. That feature may find applicability for multi-sensor devices, where the sequentially may be required only for the same sensor readings, but the lack of resources negates the possibility of opening multiple connections.
Finally, the experiments may be repeated for more constrained devices and less power-hungry wireless technologies to spot if major differences arise in a context where very tiny devices are employed.


==> thesis-sections/energy.tex <==
\section{Energy consumption for Quic and TCP}\label{chap:energy}

The first experiment campaign regards energy evaluation of \acrshort{mqtt} publish requests performed via the custom simple-client tool described in \ref{sec:client-tool}. The experiments aim to highlight possible differences between \acrshort{quic} and \acrshort{tls} over \acrshort{tcp} transport protocols by varying some parameters to compare multiple scenarios and network conditions. Note that the choice to compare \acrshort{quic} with \acrshort{tls} on top of \acrshort{tcp} stems from the fact that the new transport protocol provides by default a secure connection. In particular, the \acrshort{quic} standard requires the latest version of \acrshort{tls}, i.e. 1.3. For a fair comparison also for \acrshort{tls} on top of \acrshort{tcp} is considered the same version.

Each request sent by the client is evaluated independently of the others, establishing a new connection with the broker from scratch. Moreover, each configuration in the experiment is repeated 30 times to obtain statistically significant results. The adopted schema models a sporadic traffic generated by a node in the \acrshort{iot} network towards a collection point waiting for incoming messages. The node may adopt duty-cycle techniques to save energy in the idle periods, thus the connection can't be kept alive in the sleeping periods. Alternatively, the traffic model can also accommodate periodic traffic for which the interval between two messages is long enough to still allow the duty cycling approach.

Regarding the messages exchanged between the client and the broker, from an application perspective, the following sequence represents the entire communication for each request:
\begin{enumerate}
	\item Client sends connect message to the broker
	\item Client waits for connection acknowledgement from broker
	\item Client sends publish a message to the broker
	\item Client waits for publish acknowledgement from broker
	\item Client sends a disconnect message to the broker
\end{enumerate}

The captured energy traces include a portion of energy due to the initialization of the client, messages, and other data structures required to establish the connection. These operations have an impact on the final results, but it doesn't exceed a few percentage points in the worst case and this overhead is paid by all requests, allowing a fair comparison between different configurations. 

\subsubsection{Experiments}
The experiments to obtain the broadest possible comparison between the two transport protocols were carried out varying several parameters regarding different aspects of the communication:
\begin{itemize}
    \item \textbf{Payload size}, the size of data to transmit may have a great impact on the final results, for example, \acrshort{quic} may grant benefits over \acrshort{tls} only for small size payloads, due to the lighter connection establishment.
    \item \textbf{Network delay and bandwidth}, the different mechanisms adopted by the two protocols may offer advantages over the other only in particular network scenarios.
    \item \textbf{Access network}, access networks characterised by different properties, which could go beyond the simple difference in latency and bandwidth, may impact the comparison results. 
\end{itemize}

The quality of service adopted for these experiments is \textit{AtLeastOnce}, i.e. the sender ensures that messages are received at least once, but there is no guarantee about the possible duplication of messages received by the recipient.

\bigbreak

In \ref{tab:energy_parameter_space} a summary of explored parameter space is reported, including the technology of cellular network exploited. The access network plays a key role for \acrshort{iot} applications, in particular, the latest cellular technology 5G is a promising innovation for the domain \acrshort{iot}, thanks to its improvement in latency and bandwidth that can provide benefits for current applications and pave the way for new ones. Although cellular networks and 5G may unleash the power of the \acrshort{iot}, the energy issue must still be taken into account to avoid a short life span of battery-powered devices. The improved characteristics of 5G networks compared to the previous generation could alter the relationship between \acrshort{quic} and \acrshort{tls}, favouring one over the other. 

As will be explained below, the last two payload sizes were adopted only on a subset of experiments, while for the others the cartesian product of all parameters was considered, generating 240 configurations, plus the additional ones given by the two extra payload sizes equal to 8 configurations. All considered, the number of configurations is 248, each repeated 30 times producing a total number of experiments equal to 7440. A rough estimate of the time needed to complete an experiment, including set-up, request, and additional operations, is 45 seconds, so a rather large amount of time is needed to complete the energy evaluation campaign.

\begin{table}[!t]
	\centering
	\caption{Energy experiment parameter space}
	\begin{tabular}{lr}
		\toprule\toprule
		\multicolumn{1}{c}{\textbf{Parameter}} & \multicolumn{1}{c}{\textbf{Value}} \\
		\midrule
		Transport protocol & \acrshort{tls} (v1.3), \acrshort{quic} \\
		\midrule[0pt]
        \multirow{2}{*}{Payload size} & 128B, 1KB, 8KB, 64KB, \\ & 512KB, 1MB, 4MB, 32MB \\
		\midrule[0pt]    
		Bandwidth & 100\%\footnotemark, 5Mbit/s \\
		\midrule[0pt]
		Delay & 0ms, 20ms, 40ms, 60ms, 80ms \\
        \midrule[0pt]
        Access network & 4G, 5G \\
		\bottomrule
	\end{tabular}
	\label{tab:energy_parameter_space}
\end{table}
\footnotetext{No bandwidth restriction}

Before analyzing the results it's worth highlighting that the considered metric is the energy spent per request for the different configurations, however, the execution time was also collected. In the following, only the energy results will be reported, not only because they are the primary purpose of this thesis, but also because there is a fairly close relationship between the two metrics, i.e. the results in terms of execution time closely mirror the energy results. The similarity between metrics comes from the fact that the energy track is synchronized with the \acrshort{mqtt} request, for which the most energy-hungry phase is that of data transmission, which is also the most time-consuming operation of the entire request. The other operations required to complete the request are not computationally intensive but are limited to the construction and initialization of a few data structures that have a small impact on the final metrics. 

\subsubsection{Results}
The collection of the data took a few days as expected and produced an amount of data in the order of gigabytes, largely due to the saved power monitor tracks. In the following the collected data are analysed following an incremental approach, introducing one parameter at a time. Unless otherwise stated, all aggregate data reported refer to the median of the experiment repetitions, which is preferred to the simple mean due to its lower sensitivity to variability. Moreover, to save space the configuration in the graph legend is reported in a short form, following the convention "Access Network-Bandwidth Restriction-Additional Delay-Transport Protocol", e.g. "4G-100\%-0-quic".

\subsubsubsection{Payload size}
The first scenario under analysis is the comparison between \acrshort{tls} and \acrshort{quic} by only varying the payload size from 128 bytes to 1 megabyte over a 4G connection without artificial delays or bandwidth restrictions.

The first trials showed remarkably better results for \acrshort{tls} over \acrshort{quic} starting from a payload size of 8KB, however, a strange trend came up for the latter: the energy required to transfer an 8KB message was notably higher than the one required by a 64KB message in all the repetitions. The results are summarized in the \ref{fig:energy_payload_segmentation_on}, in which a line chart reports the energy trend (on logarithmic scale) of the two series over payload size (on base 2 logarithmic scale).

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{images/energy/energy_payload_segmentation_on_log.pdf}
    \caption{Energy over payload size (\acrshort{gso} on)}
    \label{fig:energy_payload_segmentation_on}
\end{figure}

The odd behaviour required a deeper analysis of the developed code, which pointed out that during \acrshort{quic} requests starting from a payload of 8KB, an error is generated before the successful completion of the requests. Such error is caused by the kernel optimization \acrfull{gso}, not supported by the \acrshort{rpi} system, but used by client-tool. The optimization was recently introduced in the Linux kernel to improve the transmission of large packets by reducing the processing overhead by delaying packet fragmentation as much as possible to meet the network-compliant \acrshort{mtu}. The Linux kernel installed on the \acrshort{rpi} doesn't support the \acrshort{gso}, but the \acrshort{quic} implementation adopted by the client tool is not able to obtain this information in advance, so it tries to send the message leveraging the optimization, producing an error that will require the transmission with the optimization disabled. Although the mechanism can complete the request regardless of kernel support, the dynamic fallback to a standard transmission requires time and energy that affect the final results, degrading \acrshort{quic}'s performance. To overcome the problem introduced by the lack of support to the \acrshort{gso}, it was manually disabled during the configuration of the \acrshort{quic} connection in the client tool, removing the initial attempt that produced the error.

Disabling the optimization in the client tool allowed a fair comparison between the two transport protocols and the new data showed completely different results, dramatically improving \acrshort{quic}'s performance. The new results, plotted in \ref{fig:energy_payload_log}, follow a monotonically increasing trend for both curves, as expected by increasing the payload size. The other aspect that deserves to be highlighted is that \acrshort{quic} obtains better results for any payload size, in contrast to previous comparisons between the two transport protocols. It is important to quantify the magnitude of the difference in the results, so taking a look at the data, reported in tabular form in \ref{tab:energy_payload}, it is clear that the largest differences appear for small size payloads, and then tend to shrink. 

\begin{table}[!t]
    \caption{Energy over payload size}
    \centering
    \begin{tabular}{rrrr}
    \toprule\toprule
    \multicolumn{1}{c}{\textbf{Size}} & \multicolumn{1}{c}{\textbf{\acrshort{tls} [mJ]}} & \multicolumn{1}{c}{\textbf{\acrshort{quic} [mJ]}} & \multicolumn{1}{c}{\textbf{Difference [mJ]}} \\
    \midrule
    128B & 1103.01 & 999.32 & 103.69 \\
    \midrule[0pt]
    1KB & 1114.59 & 1006.41 & 108.18 \\
    \midrule[0pt]
    8KB & 1148.97 & 1043.15 & 105.82 \\
    \midrule[0pt]
    64KB & 1617.34 & 1512.54 & 104.80 \\
    \midrule[0pt]
    512KB & 4166.70 & 4149.89 & 16.81 \\
    \midrule[0pt]
    1MB & 5260.67 & 5255.82 & 4.85 \\
    \midrule[0pt]
    4MB & 14350.90 & 14226.81 & 124.09 \\
    \midrule[0pt]
    32MB & 70302.62 & 68580.10 & 1722.52 \\
    \bottomrule
    \end{tabular}
    \label{tab:energy_payload}
\end{table}

To better investigate the differences between the two curves as the payload size increased, two more points were added (4MB, 32MB), but contrary to expectations, the difference between \acrshort{quic} and \acrshort{tls} stopped shrinking. 
The fluctuation of differences at larger payload sizes is reasonably due to the higher variability, observed in \ref{fig:energy_payload_box_partial}, which influences the results, but what can be concluded is that \acrshort{quic} is not only able to provide benefits for small payloads, but even for larger payloads, performance is no worse than \acrshort{tls}.

\begin{figure}[!t]
    \begin{minipage}[b]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/energy/energy_payload_log.pdf}
        \subcaption{Energy over payload size trend}
        \label{fig:energy_payload_log}
    \end{minipage}\\
    \begin{minipage}[b]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/energy/energy_payload_box_partial.pdf}
        \subcaption{Energy over payload size boxes}
        \label{fig:energy_payload_box_partial}
    \end{minipage}
    \caption{Energy over payload size (\acrshort{gso} off)}
\end{figure}

Note that from now on all the data displayed were obtained with the optimization disabled, so they represent a fair comparison between \acrshort{quic} and \acrshort{tls}.

\subsubsubsection{Additional delay}
The results shown so far are related to a realistic network scenario characterized by good connectivity but can be interesting to analyze the comparison in a more hostile environment, which is a common scenario for a large class \acrshort{iot} applications.
Setting up a real hostile environment may require a large effort and limit the control over the experiments, producing results that cannot be easily interpreted. For these reasons a different approach, based on artificial delay is adopted, guaranteeing precise control of the network conditions. The delay is set via the \acrfull{tc} Linux command on the broker side, forcing a configurable value for each incoming and outgoing packet. Note that the artificial delay is applied in both directions, so the \acrshort{rtt} is affected by twice the set value.

The analysis of data produced varying both payload size and delay shows a progressive improvement of \acrshort{quic} over \acrshort{tls} for higher delays and thus worse network conditions. The trends of the curves are similar to the one above described, but the differences are larger between the two transport protocols. In particular, from \ref{fig:energy_payload_delay} is possible to notice that for high values of delay, there are some overlapping or intersections between \acrshort{quic} and \acrshort{tls} curves of different configurations, i.e. sometimes \acrshort{quic} with higher additional delay can perform better (or at least equal) than \acrshort{tls} with lower additional delay, highlighting the benefits introduced by \acrshort{quic} in high-delay networks. 

Another effect of the additional delays worth mentioning is that on the variability of energy measurements. For \acrshort{quic} experiments, the variability is rather stable for each configuration, but for \acrshort{tls} higher delays generate higher variability. In \ref{fig:delay_variability} such an effect can be visualized by observing the increasing height of the boxes for requests of 1MB payload size and different additional delays.

\begin{figure}[!t]
    \begin{minipage}[b]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/energy/energy_payload_delay.pdf}
        \subcaption{Energy over payload size trend for different delays}
        \label{fig:energy_payload_delay}
    \end{minipage}\\
    \begin{minipage}[b]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/energy/delay_variability.pdf}
        \subcaption{Energy over additional delay for 1MB payload size}
        \label{fig:delay_variability}
    \end{minipage}
    \caption{Energy adding delays}
\end{figure}

For the sake of completeness, strange behaviour when comparing curves with and without additional delays is reported in \ref{fig:energy_payload_delay_comparison}. What can be inferred from the comparison is that for high payload size the energy required to complete a \acrshort{mqtt} request is lower for the configuration with additional delay (20ms) even though the execution time is higher as shown in \ref{fig:exec_time_payload_delay_comparison}. This strange behaviour is valid for both transport protocols when the payload size is 512KB and only for \acrshort{quic} for a payload size of 1MB. 

\begin{figure}[!t]
    \begin{minipage}[b]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/energy/energy_payload_delay_comparison.pdf}
        \subcaption{Energy comparison}
        \label{fig:energy_payload_delay_comparison}
    \end{minipage}\\
    \begin{minipage}[b]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{images/energy/exec_time_payload_delay_comparison.pdf}
        \subcaption{Execution time comparison}
        \label{fig:exec_time_payload_delay_comparison}
    \end{minipage}
    \caption{Delay comparison}
\end{figure}

The explanation is hard to find because several factors may have altered the results, starting with the fact that the data of the two configurations were collected on different days and therefore the conditions may not be perfectly equal. The script described in \ref{chap:setup} includes some AT commands that retrieve information about the cellular network before and after the \acrshort{mqtt} request, from which is possible to find out the cell to which the client is connected, the operative frequency and signal strength. In \ref{tab:cellular_metrics} some data about the AT commands output are reported, and the values are aggregated considering the mean due to the low variability of collected metrics. From these data, it can be observed that experiments with delays are characterized by slightly better signal quality, as stated by the \acrshort{rssi} metric. Moreover, it is interesting to note that approximately 20\% of the requests in the experiments with delays were completed using a different frequency band, which could theoretically guarantee different values in terms of energy and transfer rate. Note that the requests that were completed using another frequency band are consecutive, which means that for a certain period, the selected frequency band was that one. Due to the random ordering of the configurations, it is legitimate to consider a 20\% of iterations for each configuration performed using a different band. Regarding the experiment with delays isolating the quality signal metrics for the two frequency bands, the results show that the latter (band-3) provides even better quality, with the \acrshort{rsrp} being -94.5 dBm compared to 97.3 dBm for the former frequency band (band-7). 

The performance of the energy metric by dividing the delay curve into the two frequency bands, as shown in \ref{fig:frequency_comparison}, is very interesting. The overall trend is rather similar to the aggregated one, however, it can be concluded from the last two points that the different frequency band has a significantly positive impact on energy consumption. The still open question is how much the results depend on signal quality rather than on other hidden network factors that are not tracked by the simple information retrieved via the AT commands.

\begin{table}[!t]
    \centering
    \caption{Cellular network metrics for delay and no delay experiments}
    \begin{tabular}{lrr}
        \toprule\toprule
        \multicolumn{1}{c}{\textbf{Metric}} & \multicolumn{2}{c}{\textbf{Experiment}} \\ 
        & \multicolumn{1}{c}{\textit{\small{Without Delay}}} & \multicolumn{1}{c}{\textit{\small{With Delay}}} \\ 
        \midrule
        Cell ID & 101 & 101 \footnotemark{} \\ 
        \midrule[0pt]
        & & EUTRAN-BAND7 \small{(1119)} \\  
        \acrshort{lte} Band & EUTRAN-BAND7 & EUTRAN-BAND3 \small{(321)} \\  
        \midrule[0pt]
        \acrshort{rssi} & -65.40 dBm & -64.80 dBm \\
        \midrule[0pt]
        \acrshort{rsrp} & -99.30 dBm & -96.90 dBm \\ 
        \bottomrule
    \end{tabular}
    \label{tab:cellular_metrics}
\end{table}
\footnotetext{Except one request}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{images/energy/energy_frequency_comparison.pdf}
    \caption{Frequency band comparison}
    \label{fig:frequency_comparison}
\end{figure}

\subsubsubsection{Bandwidth restriction}
The same consideration of network conditions applies to bandwidth, for which a lower transfer rate can legitimately be expected in \acrshort{iot} applications. The limit is set again via \acrshort{tc} command on the broker-side, imposing both a download and upload rate limit, i.e. for incoming and outgoing data, moving the bottleneck of the network on the broker-side instead of on the client access network. The value of the symmetrical limit, i.e. equal in both directions, was chosen by setting a fairly tight constraint on the bandwidth, keeping about one-fifth of the original download bandwidth.

Initially, the limit was erroneously set only on the upload direction, thus from the client's point of view on its download bandwidth. This limit did not produce any appreciable difference in the results, which indeed appear better than those without bandwidth limitation, probably for the same reasons analyzed in the delayed case. Reasoning about the communication scheme, the results of the first attempt should not be surprising, because the significant part of the data transfer occurs from the client to the broker, i.e. upload from the client's point of view and download for the broker, that is the direction not affected by the bandwidth restriction. The limit was only imposed on acknowledgements, consisting of a few bytes, sent by the broker in response to messages from the client.

The results obtained by correctly setting the restriction on both communication directions resemble those without restriction only for small payload sizes, which can be justified by the fact that for a low amount of data, the actual data transfer is not the predominant part of the communication, which is instead dominated by delays. On the other hand, for payload sizes in the order of megabytes, the difference between bandwidth restriction and no restriction is clear, as can be visualized in \ref{fig:energy_bandwidth_comparison}. Note that the same considerations apply when introducing additional delays in configurations, simultaneously imposing constraints on both delay and network bandwidth.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{images/energy/energy_bandwidth_comparison.pdf}
    \caption{Energy over payload size bandwidth comparison}
    \label{fig:energy_bandwidth_comparison}
\end{figure}

Regarding large payload sizes, the results show an interesting difference for which the performance of \acrshort{tls} seems to be slightly better than that of \acrshort{quic}, reversing the trend obtained so far. Again, it is necessary to quantify the order of magnitude of the difference, and as can be observed from \ref{fig:energy_band_large_payload_comparison}, the two results are very close and it is not possible to state which is better than the other. However, these results prove once again that \acrshort{quic} can obtain performance comparable to \acrshort{tls} even when the size of payloads is quite large. 

Finally, although the \ref{fig:energy_bandwidth_comparison} the plot scale does not allow for an accurate comparison for small payload sizes between the restricted and unrestricted data, it should be pointed out that the restricted results tend to stay under the unrestricted ones, i.e. they have slightly better energy consumption. The cause of these unexpected results is not easy to attribute, however, the same AT log analysis performed for the data with additional delays shows again that the signal quality is generally better for the results collected under the bandwidth restriction configuration.  

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{images/energy/energy_bandwidth_comparison_large_payload.pdf}
    \caption{Energy comparison between bandwidths for large payload sizes}
    \label{fig:energy_band_large_payload_comparison}
\end{figure}

\subsubsubsection{Access network}

The results obtained from changing the cellular technology don't alter the comparison between the two transport protocols. The differences between the two curves are more evident introducing the same network constraints already described above. In \ref{fig:energy_5G} only a subset of curves is reported to simplify the analysis and visualize the trend just described.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{images/energy/energy_5G.pdf}
    \caption{Energy over payloads for 5G access network}
    \label{fig:energy_5G}
\end{figure}

Another interesting analysis of the 5G configuration is the comparison with the data collected from the same experiments in the 4G version. The expected conclusion is a supremacy of the new technology, at least in terms of execution time, over the old, but the results depict a very different scenario. Even the additional payload size (4MB and 32MB), added to the comparison to ensure that the higher bandwidth of 5G only shows its advantages for a considerable amount of data to be transferred, doesn't gain any advantages over the old technology. In \ref{fig:energy_4G_5G_comparison} the results are reported and from the interweaving of lines, it's clear that the improvements provided by the new technology don't produce the expected results. The comparison is even worse for 5G once network constraints are introduced, but in this case, the motivation is largely due to the fact that by imposing artificial limits on the network, the strengths of the new technology are lost.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{images/energy/energy_4G_5G_comparison.pdf}
    \caption{Cellular technologies comparison}
    \label{fig:energy_4G_5G_comparison}
\end{figure}

Although the results of the 5G configurations didn't meet expectations, it's fair to point out that the experiments were characterized by several problems that might have compromised the results:
\begin{itemize}
    \item \textbf{Provider network infrastructure}, the 5G infrastructure available is a mixed mode of new and previous technology, created to speed up the deployment of 5G by exploiting the 4G infrastructure already in place. Hybrid technology is referred to as 5G \acrfull{nsa} and cannot fully guarantee the benefits promised by full 5G technology. 
    
    \item \textbf{Network availability}, the 5G network coverage is still limited to some areas and the location from which the tests are launched cannot guarantee stable 5G connectivity. When the network interface detects a poor 5G signal, it downgrades the connection from 5G to 4G autonomously, without the possibility of keeping track of the status of the network. Such behaviour is quite annoying because it doesn't guarantee that a request is actually completed using a 5G network, raising doubts about the interpretation of the collected data.
\end{itemize}

Please note that such considerations are related to the time of testing and for the adopted network provider, the situation may change rapidly in the future.

As already mentioned, network status monitoring is not continuous, the network card does not provide any means to ensure that a 5G connection is not downgraded to 4G, so the best that can be done is to check before and after the \acrshort{mqtt} request if the 5G connection is available. The check is not exhaustive because it cannot provide information on what happens in between, so the information is only indicative and should be taken with a grain of salt. Once the entire scenario has been described, it's not possible to give any conclusions for 5G configurations because the data can't guarantee that refers to an actual 5G connection and not to a mixed mode between different network generations. 


==> thesis-sections/introduction.tex <==
\section{Introduction}\label{chap:introduction}

The \acrfull{iot} is a concept that describes the network of interconnected physical objects, empowered by electronic devices able to provide computational and communication capabilities and often equipped with sensors and actuators to interact with the surrounding environment \cite{atzori2010internet}-\cite{rose2015internet}. These devices can communicate and exchange data with either local or remote devices through the network, enabling them to collect and analyse information sensed in the working environment and to perform actions autonomously without human intervention. Nowadays, \acrshort{iot} has moved from an emerging paradigm to an established one, nonetheless the widespread diffusion is not expected to slow down, further increasing the number of interconnected devices deployed across a wide range of environments, such as industries, cities, rural areas, buildings, etc. The presence of surrounding \acrshort{iot} devices, which can be considered a complete system, may go unnoticed, thus integrating supporting tasks without explicit intervention into people's lives, fueling the so-called pervasive computing paradigm. A common application of \acrshort{iot} systems is in the automation field, for which the use of sensors and actuators in the controlled environment allows for taking autonomous decisions based on distributed application logic that relies on the collected information.\cite{Breivold2015:internet}-\cite{Tokognon2017:structural}. Automation finds application across diverse contexts, ranging from regulating heating and lighting to safety-critical tasks characterised by very strict requirements. 

In general, those systems can be referred to as monitoring and controlling systems for which the freshness of data engaged in decision-making often assumes a pivotal role. Such requirement is usually stressed by the distributed nature of the systems, which require the exchange of data through the network adding some latency to the flow of information. The problem can be exacerbated by the current trend of employing cloud technologies to host some application components that are not implemented on devices, such as the data collection point and control logic. These components are often structured following a micro-services architecture, which is suitable for leveraging cloud resources and simplifying the development process. This model introduces a spatial separation between application components and thus a latency increase in the inter-component communications. Application dispersion represents just one aspect influencing communication latency, with various other factors playing significant roles. Among them, the access network constitutes a substantial contributor to latency. Various network technologies can be applied in \acrshort{iot} systems, but often a not negligible effort is required to set up the appropriate infrastructure. For example, the WiFi technologies, or constrained versions of them, that could be adopted in various scenarios, require the installation of access points. However, there are some cases in which is not feasible or convenient to install a dedicated infrastructure, such as for systems deployed in rural areas. For this sub-group of \acrshort{iot} systems, the cellular infrastructure that has already a widespread diffusion could be a cost-effective solution. 

The freshness of data can be measured through the \acrfull{aoi}, a metric that gained popularity in the \acrshort{iot} context due to its simplicity and effectiveness \cite{kosta2017age}-\cite{yates2021age}. The \acrshort{aoi} can be described as the time elapsed since the last update, i.e. its value in time is given by the difference between the generation timestamp of the latest data received and the current time. 

In the \acrshort{iot} context, devices are predominantly battery-powered, so ensuring optimal performance of metrics such as data freshness becomes tied to managing the limited energy resources available, which represent the most strict constraint. Therefore, any efforts to enhance data freshness must cope with the constraint of energy availability, also taking into account that battery replacement is often not possible, so battery life must be extended as much as possible. Communication represents a substantial portion of the overall energy consumption throughout the life cycle of a device, and network technology once again assumes a central role. Regardless of whether the technology is more or less energy-intensive, the usage pattern represents one of the main factors determining the energy spent on communication activities. In particular, the adopted application protocol can determine a different level of intensity in the usage of the resources available to the device, directly reflecting on the energy consumption attributable to communication. The choice and configuration of the communication protocol represent a key factor in keeping energy consumption under control, acting on the software side and thus ensuring good flexibility in system design.

\acrfull{mqtt} \cite{mqtt-v3r1}-\cite{mqtt-v5.0} is one of the most adopted application protocols in monitoring and controlling systems and in general in the \acrshort{iot} domain. The protocol follows a publish-subscriber paradigm, setting up indirect communication between the communication ends leveraging the presence of an intermediary broker and an organization of messages categorized by topic. The \acrshort{mqtt} standard requires the application protocol to run on top of a reliable transport layer. The de-facto standard for a reliable transport layer is \acrfull{tcp}, originally designed for wired networks in an era in which network security was not a requirement. Nowadays, the pervasive nature of devices leads to increasing attention on the privacy of the collected data that may carry out sensitive information about the system and the users. The solution to address the lack of privacy and security is achieved by transforming a simple \acrshort{tcp} connection into a \acrfull{tls} connection, which can protect the data sent over the network.

The rapid evolution of networks has necessitated the adoption of trade-offs to cope with the new requirements, however, a challenge arises in continuing to rely on \acrshort{tcp}, whose evolution struggles to keep pace with the network evolutions. To cope with this impasse new protocols have been proposed, even if they have often encountered obstacles due to the dominant position of \acrshort{tcp}. To avoid the problems arising from \acrshort{tcp}, the solution has been to adopt an unreliable transport layer, i.e., \acrfull{udp}, whose standardisation is comparable to that of \acrshort{tcp}, and to implement the reliability mechanism at the application level. Originally the usage of \acrshort{udp} was limited for applications where message reliability was secondary to performance, minimizing the overhead of the transport layer. This solution has a clear limitation in the process of developing new application protocols that must provide a mechanism that should not be a problem addressed at that level. The Quic protocol \cite{rfc9000} exploits the same concept and starting from \acrshort{udp} realizes a complete transport protocol that can be adopted by the upper layer while keeping the reliability mechanism transparent. In addition, the recent introduction of \acrshort{quic} imposes some requirements to be faced by the protocol, including the security issue handled via the most recent version of \acrshort{tls} directly integrated into the transport protocol connection. \acrshort{mqtt} can run on top of \acrshort{quic} since the requirement of reliability is met and also the additional requirement on security, which would require a dedicated \acrshort{tls} session on top of \acrshort{tcp}, is granted by the new protocol. The \acrshort{quic} transport protocol can potentially guarantee some improvement, such as a streamlined connection establishment, that may fit better in a context where computational resources are constrained.

This thesis presents a combined experimental study of energy and \acrshort{aoi}, framed within an \acrshort{iot} scenario primarily focused on monitoring and controlling any system that requires a certain level of data freshness. The network technology under study is cellular, specifically 4G, but also 5G in some configurations. The protocol analyzed is \acrshort{mqtt}, which is quite common in these scenarios, both in its standard version, leveraging the secure variant over \acrshort{tls}, and on top of the emerging transport protocol \acrshort{quic}. The study proposes two types of experiments. The first type evaluates individual requests solely from an energy perspective, primarily to assess the suitability of the \acrshort{quic} protocol within this context. The second type constitutes the combined study, where both metrics are assessed over a defined time window during which multiple requests are transmitted at a predetermined rate. Both experiments consider a range of parameters, including message payload sizes and artificially modified network conditions. An experimental approach is adopted for the collection of data in both experiments, measuring the energy directly using a power monitor physically attached to the device under test that transmits messages on the Internet through a real cellular network.

==> thesis-sections/setup.tex <==
\subsection{Setup}
The experimental evaluation of the metrics of interest required a setup composed of multiple hardware and software components. The client side, i.e. the publisher in the \acrshort{mqtt} terminology, is installed on a \acrfull{rpi} board, that acts as an \acrshort{iot} device. This device is equipped with a cellular network card \cite{cellular-hat} able to support both \acrfull{lte} and \acrfull{ng} communication technologies. The requests sent by the client are directed towards an \acrshort{mqtt} broker hosted by a server in the University of Pisa cloud. The device represents a battery-powered device, but to evaluate the energy required to complete the requests under test it is powered by a power monitor. A power monitor is a device able to offer a configurable power source and record the total energy supplied during its activity. The adopted power monitor is the Otii Arc Pro from Qoitech \cite{otii}. The main features of this instrument are the easy-to-use software \acrshort{api} to control the energy recording and the serial \acrfull{uart} interface that can be exploited both to send commands to the device and to annotate the recorded trace with timestamps to precisely confine the portion of the total energy required during the execution of an experiment. The software control of the power monitor requires an \acrshort{usb} connection with a laptop that acts as a controller for the experiments executed on the \acrshort{rpi}. The base configuration is composed of four hardware devices, each one running a different software component:
\begin{itemize}
    \item \textbf{\acrlong{rpi}}, is the \acrshort{iot} device under test on which data is generated and sent using the \acrshort{mqtt} protocol with a set of given parameters.
    \item \textbf{Server}, hosts the broker to which requests from the device under test are directed.
    \item \textbf{Power monitor}, is responsible for measuring the energy required by the device during the execution of the experiments.   
    \item \textbf{Laptop}, represents the controller of the experiments, provides the parameter of each configuration to the \acrshort{rpi} and controls the power monitor via dedicated \acrshort{api}.
\end{itemize}

To evaluate only the energy consumption of the device the experimental setup above described would be sufficient, but in this thesis also the \acrshort{aoi} is considered and it requires some additional pieces for a proper evaluation. The setup needs another client acting as a subscriber for the data produced by the \acrshort{rpi}. The subscriber is placed on the laptop and after the subscription with the broker it is in charge of computing the time difference between the instant when the message was generated and the instant when it was received. The laptop is connected to the university network via a WiFi access network and can reach the server without passing through the public Internet, so the network segment delay between the server and the publisher is rather small. The overall configuration corresponds to a rather common scenario in the \acrshort{iot} domain, in which the \acrshort{rpi} acts as a device installed somewhere that produces data, typically collecting information by monitoring the environment. The subscriber on the laptop in turn can be considered as a cloud application that deals with the collection of the data produced, applying logic that may be sensitive to the freshness of the information obtained from the data. The two parties exchange information through the broker, hosted in the cloud as the subscriber, which represents a centralized entity enabling indirect communication according to the \acrshort{mqtt} protocol.

The only missing aspect is the time synchronization mechanism between publisher and subscriber, required to obtain a meaningful result from the difference between the two timestamps, needed for the \acrshort{aoi} computation, the first one recorded on the \acrshort{rpi} and the second one recorded on the laptop. Synchronizing clocks of devices without any specialized hardware module such as \acrshort{gps} receiver, is not an easy task. The adoption of the \acrfull{ntp} protocol may be a cost-effective solution, but two major problems arise:

\begin{itemize}
    \item The \acrshort{rpi} and the laptop have assigned dynamic private addresses, so they are hidden behind the \acrshort{nat} mechanism and are not reachable from external hosts.
    \item The connection between the two clients can only be established through the public Internet, which introduces a level of instability in communication delays.
\end{itemize}

Although the lack of direct addressing can be resolved by adopting some port forwarding services, such as the one offered by Ngrok \cite{ngrok}, the need to traverse the public Internet limits the accuracy of synchronization, especially in the case of asymmetrical connections. The solution adopted for clock synchronization is based on the fact that, even though the two clients are separated by the public Internet network, they are physically in the same place and a second connection can be established via an Ethernet cable, building up a \acrfull{lan} without any intermediary between the two nodes that are directly connected. The \acrshort{ntp} protocol can exchange messages via the Ethernet interface, while the data transmitted by the experiments will follow the path in the public Internet reached via the cellular network.
The \acrshort{ntp} protocol is based on a hierarchical client-server model, where the client synchronizes its clock with the time-reference server in the lowest level of the hierarchy. The server of the last level in turn synchronizes its clock with the server in the upper level, and so on up to the first level, which can be a very high-precision atomic clock. Regarding the experimental setup the \acrshort{rpi} represents the final \acrshort{ntp} client, while the laptop is the time-reference server in the last level. More details about \acrshort{ntp} protocol and the configuration steps required to enable the time synchronization are reported in the appendix \ref{sec:clock_sync}.

Some technical specifications on the hardware used in the setup are reported in \ref{tab:hardware}, while the values for the \acrshort{rtt}, the throughput and hops in the path of the most relevant connections are given in \ref{tab:net_stats}. The \acrshort{rtt} was collected by repeating multiple times the "ping" command, available both on the \acrshort{rpi} and the laptop, while for the throughput, both upload and download, was employed the "iperf3" tool \cite{iperf}. Given the fact that the communication flows mainly from publisher to broker and from broker to subscriber the most relevant throughput direction is upload for connection \acrshort{rpi}-server and download for connection laptop-server. The number of hops has been derived through the "tcptraceroute" command on the \acrshort{rpi} and the "tracert" on the laptop, both based on incremental \acrshort{ttl} field in the \acrshort{ip} datagram sent toward the destination host.


\addtocounter{footnote}{-2}
\stepcounter{footnote}\footnotetext{The processor has four cores, but only one is enabled to reproduce a resource-constrained device faithfully}
\stepcounter{footnote}\footnotetext{The server is a virtual machine that can benefit from only 2 cores out of a total of 14 available}

Finally, a view of the entire setup is shown in the diagram of \ref{fig:setup_overview}, in which are highlighted the connections between the three devices and the path followed by data transmitted in the experiments.



\subsection{Automation Script}
The experiment campaigns planned to collect all the necessary data for the study include many configurations, making it difficult to manually run one trial at a time. Moreover, in addition to the time-consuming tasks a manual approach would risk producing some errors, possibly biasing the data obtained. The operations to carry out are quite repetitive, so they can be easily automated via software, developing a simple script for each configuration executes the preliminary steps to launch the experiment and once completed saves the data measured and moves them to a dedicated directory. Python is the language chosen for the automation script because of its high productivity, ease of use and wide support. The automation script is composed of two parts:
\begin{itemize}
    \item \textbf{Controller}, script running on the laptop and acting as director of the experiment campaign.
    \item \textbf{Device}, script running on the \acrshort{rpi} and acting as a simple proxy waiting for the configuration's parameters to execute.
\end{itemize}

The communication between the two sides exploits the \acrshort{uart} connection established between the \acrshort{rpi} and power monitor in turn connected to the laptop. This connection, as already anticipated, can be used to send the configuration's parameters and to annotate the power monitor trace to confine the energy portion due to the execution under test. In general, the serial connection is reliable and is not a common source of error due to its simplicity and point-to-point nature of connection. However, the serial connection established between the \acrshort{rpi} and the laptop is a little more complicated by the fact that the power monitor acts as an intermediary in the middle, transforming the initial \acrshort{uart} connection into a \acrshort{usb} one. The presence of a third device in the connection accounts for a slighter increase in the communication latency, but still in the acceptable order of a few milliseconds. The bothersome problem is that the connection has proven unreliable, introducing some errors in the exchanged messages from time to time. The errors appear sporadically, probably due to some strange behaviours internally to the power monitor, and to cope with them initially a \acrfull{rdt} mechanism was introduced in the script. The mechanism included a simple, but comprehensive, \acrfull{arq} scheme that, while able to solve the unreliability problem, introduced an additional source for potential errors in the script, originating from exceptional situations not considered. In the final version of the script, the \acrshort{arq} mechanism was shelved in favour of a different approach, based on the repetition of the entire configuration in case of message corruption. Although this approach may seem inefficient the error frequency is quite low and occurs only from the \acrshort{rpi} to the laptop. Each transmitted message is protected by a simple \acrshort{crc} and when the controller receives a corrupted message restart the failed configuration.

The operations in charge of the controller scripts are the following:
\begin{itemize}
    \item Read the configuration file containing the parameters for the experiment campaign.
    \item Launch the \acrshort{mqtt} subscriber and register it to the broker on the configured topic.
    \item Establish a connection with the power monitor and consequently the \acrshort{uart} connection with the \acrshort{rpi}.
    \item For each configuration in the experiment campaign the following sub-tasks are executed:
    \begin{itemize}
        \item Enforce possible network constraints on the broker side, e.g. bandwidth restriction and additional latency.
        \item Start recording energy trace.
        \item Send the parameters through the serial connection to the \acrshort{rpi}.
        \item Wait for start and stop messages from the \acrshort{rpi} and concurrently receives messages for the \acrshort{aoi} computation.
        \item Once the configuration is completed the energy trace is stopped and the portion associated with the experiment is extracted.
        \item Download metrics collected on the device from an intermediary server and jointly to the data captured locally save them in the appropriate directory.
    \end{itemize}
\end{itemize}
Note that the subscriber is the component in charge of receiving the messages published by the \acrshort{aoi}, thus representing the final receiver for the \acrshort{aoi} computation. If any of the above steps fails the configuration is autonomously restarted.
\bigbreak
Regarding operations in charge of the device scripts are the following:
\begin{itemize}
    \item Waiting for configuration parameters on \acrshort{uart}.
    \item Force synchronization with the laptop.
    \item Set the desired cellular technology.
    \item Extract some statistics on network quality.
    \item Send start message via \acrshort{uart}.
    \item Launch the configuration with the proper parameters.
    \item Send stop message via \acrshort{uart}.
    \item Upload the metrics collected locally on an intermediary server.
\end{itemize}
In case of failure of one of the above steps, the device informs the controller with a special error message, triggering the restart of the failed configuration.

\subsection{Client tool and Broker}\label{sec:client-tool}
The experiments about \acrshort{mqtt} requests require two main software components:
\begin{itemize}
    \item \textbf{Client}, is the software responsible for publishing or subscribing to the broker.
    \item \textbf{Broker}, it is the software that acts as an intermediary between publishers and subscribers to forward all messages on a given topic to all subscribers who have subscribed to that topic.
\end{itemize}

Support for the \acrshort{mqtt} protocol is very broad, there are many libraries available to integrate this communication protocol into applications running on different platforms, from tiny embedded devices to powerful servers, usually offering implementations for a wide range of programming languages. One of the most common libraries is Eclipse Paho \cite{paho}, which offers a very large set of implementations correlated with clear documentation for its use. The problem encountered in carrying out the experiments in this thesis stems from the fact that the \acrshort{mqtt} protocol was designed on top of the \acrshort{tcp} transport protocol. Almost all libraries focus on the standard specification, at most providing some additional functionality on top of \acrshort{tcp}, such as secure connections via \acrshort{tls} or web technologies like \acrfull{ws} or \acrfull{wss}.
The same considerations apply to the broker: many implementations are available, but among them only a small subset offer support for the \acrshort{mqtt} protocol over the \acrshort{quic} transport layer. For instance, Eclipse Mosquitto \cite{mosquitto}, which is a commonly adopted broker, limits its support to only the transport layer \acrshort{tcp} and the variants mentioned above. The search for a broker with \acrshort{mqtt} over \acrshort{quic} led to EMQX \cite{emqx}, an open-source implementation offered by the EMQ group, a company that provides the infrastructure required by the cloud component of \acrshort{iot} applications. The EMQX broker fulfils all the requirements for the experiments designed for this thesis, allowing an easy configuration and deployment of the broker on the server in the University of Pisa cloud, and even if no client library is shipped together with the broker, EMQ itself offers two implementations with \acrshort{quic} support as separate projects, i.e. NanoSDK \cite{NanoSDK} and Emqtt \cite{emqtt}. The implementations that have been tested are reported in \ref{tab:client_lib}. 
\begin{table}
    \centering
    \caption{\acrshort{mqtt} client libraries}
    \begin{tabular}{lllll}
    \toprule\toprule
    \multicolumn{1}{c}{\textbf {Library name}} & \multicolumn{1}{c}{\textbf {Language}} & \multicolumn{1}{c}{\textbf {\acrshort{quic} implementation}} & \multicolumn{1}{c}{\textbf{Author}} & \multicolumn{1}{c}{\textbf{Problem}}\\ 
    \midrule
    NanoSDK & C & MsQuic & EMQ & Building problems\\
    \midrule[0pt]
    Emqtt & Erlang & Quicer (MsQuic wrapper) & EMQ & Poor performance \\
    \midrule[0pt]
    Rumqtt & Rust & Quinn & Bytebeam & Bug in the software \\
    \bottomrule
    \end{tabular}
    \label{tab:client_lib}
\end{table}

\subsubsection{NanoSDK}
The first implementation tested was NanoSDK, an extension adding \acrshort{mqtt} support for the broader library NNG \cite{NNG}, which in turn is a modern re-implementation of the older Nanomsg \cite{NanoMsg}, originally developed to support a wide range of communication patterns. The entire chain of libraries is developed by adopting C language for performance reasons. The \acrshort{mqtt} protocol, introduced in NanoSDK, supports both \acrshort{tls} on top of \acrshort{tcp} and \acrshort{quic}. The \acrshort{tls} implementation adopted in the project is WolfSSL \cite{wolfSSL}, optimized for constrained systems, while for the \acrshort{quic} implementation, the adopted one is MsQuic \cite{msquic}, and open-source project maintained by Microsoft and based on a customized version of the common OpenSSL for the cryptography component. The project offers also some wrappers for high-level languages, such as Java and Python, however, despite the promising approach the usage of the library encountered some problems in the preliminary tests. The library, despite the successfully compilation, crashed during the running of some tests on \acrshort{quic} protocol, the protocol that motivated its usage. After some tests, the library was discarded due to the time-demanding process of debugging, exacerbated by the complex dependencies formed by the interaction of multiple software projects.

\subsubsection{Emqtt}
The second implementation tested was Emqtt, developed by adopting the Erlang programming language. The unpopular choice of programming language stems from the fact that also the EMQX broker is implemented by leveraging the same technologies, ensuring in this way a full ecosystem able to guarantee perfect interoperability without any additional effort. Moreover, the nature of Erlang, a purely functional language designed for distributed systems, fits well with networking operations. The drawback is that Erlang is not a compiled language, but it needs a runtime to interpret a high-level bytecode generated directly by the source files. The cope with this issue the core components are wrapped in the Erlang code and implemented by faster languages, such as the \acrshort{quic} library that is based once again on MsQuic. The workaround enables achieving acceptable performance when the software operates on a system with moderate resources. However, significant performance degradation occurs when executing the code in a constrained environment. This issue becomes pronounced when the execution flow involves only a single published message. The penalty imposed by the runtime during software boot consumes a substantial portion of the program's execution time, thereby distorting the collected results, especially concerning energy consumption. The preliminary tests using the Emqtt client for the \acrshort{mqtt} tool showed execution times in the order of seconds, thus making it impossible to proceed with the study employing this library.

\subsubsection{Rumqtt}
The Bytebeam's Rumqtt project \cite{rumqtt} provides a full ecosystem for \acrshort{mqtt}, both broker and client library, realized through the emerging Rust \cite{rust} programming language. 
Rust is a modern, systems programming language known for its emphasis on safety, speed, and concurrency. The main feature is the new mechanism for dynamic memory management, based on some rules enforced during at developing time to move at compile time all the burden of deallocation, defining in this way a safe memory management that is not demanded by the developer and at the same time doesn't involve a runtime environment that would limit the performance. 

All the dependencies of the project are Rust-native, keeping the management and building of the library quite easy. \acrshort{quic} is not originally provided by the project, however, the support was added by a community effort and for now is available as a fork of the main code repository \cite{rumqttquic}. In \ref{fig:rumqtt-dep} an overview of main dependencies is reported. The libraries at the core of the project are mqttbytes \cite{mqttbytes} for the \acrshort{mqtt} message format, Rustls \cite{rustls}, a complete Rust implementation of \acrshort{tls}, for the cryptography components and Quinn \cite{quinn} offering support to \acrshort{quic}. Regarding the classic transport protocols, the client library offers both synchronous and asynchronous interfaces, while for \acrshort{quic} only asynchronous since the underlying library doesn't provide any other option. The lack of environment runtime offered by the Rust language would require an implementation of the underlying connection in the application, however, some libraries can relieve the developer from that burden. The library adopted in the project is Tokio \cite{tokio}, the most popular choice to exploit asynchronicity in Rust. 
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/setup/dependency_scheme.pdf}
    \caption{Rumqtt library dependencies}
    \label{fig:rumqtt-dep}
\end{figure}

The preliminary test of Rumqtt libraries provided promising results, both on usability and performance on the \acrshort{rpi}. However, some compatibility problem arises between the different \acrshort{quic} implementations on the client side and the broker, recalling that the chosen one was EMQX. After some debugging process, the problem was confined to the initial connection establishment phase, probably due to some misconfiguration. The complexity of the broker, for which the control was very limited led to the replacement of EMQX with the broker directly shipped in the Rumqtt project, named Rumqttd. The popularity of EMQX was an attractive feature to validate the setup, but taking into account that the load that will handle the broker will be quite moderate, with only one publisher and one subscriber, the new broker (Rumqttd) shouldn't account for any significant variation in the data collection.\\
The selected library allowed simple writing of the tool for publishing a message, however, during the first phase of the experiments a rather strange behaviour was identified. Varying the payload of the \acrshort{mqtt} for a given range of sizes the \acrshort{tls} configuration took a long time to complete, out of scale considering the times required by similar payload sizes. Investigating the problem showed that the application acknowledgement required by the selected quality of service was delayed by some internal component of the library and delivered only after the reception of the reply from the broker to the keep-alive mechanism of the \acrshort{mqtt} protocol. The identification of the problem allowed advancing in the debugging process, however, even after reporting the issue to maintainers and their acknowledgement of the bug the decision was to discard the client library in favour of a custom one.

\subsubsection{Custom library}
The time spent on defining the code of the first client tool based on the Rumqtt library and the good feedback encountered in the preliminary experiments until the bug was discovered, led to the idea of defining a new custom library from the same components, i.e. Rustls and Quinn for the networking part and Mqttbytes for the \acrshort{mqtt} message format. The choice of maintaining Quinn as the \acrshort{quic} implementation for the library, despite compatibility issues with the EMQX broker, stems in part from the experience already gained with this library, its ease of use and the lack of competitors showing a clear advantage, e.g. greater community support. Moreover the Rumqttd broker, unlike its client counterpart, didn't show any glaring problems during the first set of experiments.
The aim was to build a library with a well-defined interface, exposing a set of operations mapping the main functionalities offered by the \acrshort{mqtt} protocol, in such a way to reuse the tool already developed with the Rumqtt client library. The main operations needed by the experiments are:
\begin{itemize}
    \item \textbf{Connect}, the client opens a connection with the broker
    \item \textbf{Publish}, the client once connected can publish messages on a given topic
    \item \textbf{Disconnect}, the client closes the connection and the resources assigned to it can be released
\end{itemize}

In principle, a basic implementation of the \acrshort{mqtt} protocol should also provide the subscription operation to receive messages published on a given topic, but it is worth mentioning that the requirements of the developed software are those given by the energy and \acrshort{aoi} evaluation experiments that do not require the subscription operation by the \acrshort{rpi} on which the tool will run. 

\bigbreak
Regarding the implementation details the code is organized as three separate crates, i.e. in packages according to Rust's nomenclature:
\begin{itemize}
    \item \textbf{raw-mqtt-cli}, crate containing the code of the executable client tool that can be used to publish a message on a given topic according to the parameters passed via the command line. 
    \item \textbf{raw-mqtt-stream-cli}, crate containing the specific code of the executable client for the \acrshort{aoi} experiments.
    \item \textbf{raw-mqtt-lib}, library crate at the core of the project containing the implementation of the \acrshort{mqtt} protocol and exposing the interface above described.
\end{itemize}
Another key feature of the developed software that deserves to be highlighted is the asynchronous programming paradigm adopted, which has a profound impact on the architecture of the core library. The reasons behind this particular choice, which seems as an additional difficulty to cope with, originally stem from the nature of Quinn library, which was developed following this programming style. However, the asynchronous methods offered by Quinn library may in principle be wrapped in such a way to roll back to a standard synchronous interface, but it was decided to follow the asynchronous approach anyway, since network operations can theoretically benefit from this approach, optimizing the use of resources on the \acrshort{rpi}.

\bigbreak
In general, the asynchronous paradigm enables concurrent execution of tasks, allowing programs to efficiently handle I/O-bound operations, such as network requests. This model is particularly convenient in scenarios where waiting for I/O operations to complete would introduce unnecessary delays in other operations degrading performance. The idea is to split the execution flow into multiple units of work, named tasks, that may be executed in a concurrent fashion. When a task suspends waiting for a condition, e.g. network transfer to be completed, instead of blocking the entire thread another task can be executed. The modern approach to the asynchronous paradigm is based on the async/await keywords offered directly by the programming language in order to simplify the development of code. By marking functions as async, the execution flow can be suspended at points where I/O operations occur, without blocking the entire thread. When an asynchronous function encounters an await expression, if the operation cannot be completed immediately, other tasks will be executed until the awaited operation is completed. Finally, once the awaited operation finishes, the function resumes execution from the point of the await expression. From this brief introduction, the asynchronous model appears quite easy and even the burden on the developer is largely relieved by the syntactic sugar of language keywords, an underlying infrastructure needs to be set up to stop the execution of a task, schedule another and back to the first only once the awaited operation will be completed. All these operations don't come for free, especially in a programming language that doesn't involve a runtime to execute the code, for example, JavaScript where async/await keywords are available and heavily used in the context of web programming. Rust language, the one adopted, is a fully compiled language aimed to achieve high performance, thus the output of the compiler is an executable file containing machine code that can be executed without the support of a runtime. Even if the asynchronous keywords are available in principle to obtain a running program all the underlying infrastructure should be implemented following the specifications of the model provided by the language. The complexity and time required by this approach would make it impossible to develop asynchronous software, but fortunately, the concept of asynchronous runtime comes into play. The latter can be considered as a framework that takes the code containing async/await keywords and plugs it into its asynchronous infrastructure. Such operation is realized at compiling time, i.e. all the marked functions and awaited expressions are transformed to handle the suspension, scheduling and resuming of the tasks. The runtime acts as a task scheduler, similar to the system kernel scheduler with threads. The model can be emulated by adopting standard concurrent parallel programming using threads, but the significant difference is that thread management requires a non-negligible overhead in the system, which can reduce the achievable benefits. It is worth noting that asynchronous programming is best suited for I/O-related tasks, but in a computationally demanding scenario a parallel approach is still the best choice because it can take full advantage of the capabilities of the underlying hardware. However, a hybrid approach, i.e. based on multiple threads on which multiple tasks are executed asynchronously, can offer significant performance gains for many scenarios.

Tokio is probably the most used and supported asynchronous runtime for Rust, many projects are based on it including the adopted \acrshort{quic} library. Tokio offers more than a runtime because it provides many other utilities such as networking abstraction or message-passing structure to support task interactions. For these reasons also the custom library relies on Tokio both for runtime and utilities.

\subsubsubsection{Raw-mqtt-lib}
The raw-mqtt-cli is the core of the above introduced tools, offering all the required \acrshort{mqtt} operation abstracting all the underlying management of the network and the protocol itself. The adopted programming paradigm is the classic object-oriented one, which allows grouping all the network-related management into a structure, i.e. the closest concept of class in Rust, that will be used to build the other main structure of the crate that contains the logic of the \acrshort{mqtt} protocol, referred as client. The adoption of this paradigm, jointly with the use of generics, allowed smooth reuse of the same code to realize clients on top of different transport protocols, namely \acrshort{tcp}, \acrshort{tls} (v1.3) and obviously \acrshort{quic}, modifying only the network part.
Internally this crate is organized into three sub-crates, each dedicated to a specific aspect:
\begin{itemize}
    \item client, contains client structures that apply the protocol steps.
    \item network, contains the structures that allow an easy interaction with the network.
    \item utility, contains a simple command line parser to collect the parameters that can be set dynamically.
\end{itemize}

More in detail the base client structure, defined in the namesake sub-crate, is in charge of running the steps required by the protocol, which can be resumed as:
\begin{enumerate}
    \item Building a data structure containing the fields of the \acrshort{mqtt} message with the value passed by the application that uses the library.
    \item Serializing of the data structure in a protocol-compliant format.
    \item Data transmission towards the broker via an opaque network structure that hides the details of the underlying transport protocol adopted.
    \item If required reception of acknowledgement message from the broker.
\end{enumerate}

The implementation of the opaque structure, defined in the network sub-crate, is obtained by leveraging the generics concept available in Rust and similar to other programming languages. In particular, a network trait that can be considered as an interface is defined by listing the methods, return type and parameters, that must be implemented to be compliant with such trait:
\begin{itemize}
    \item \textbf{Connect}, establishes a connection with the other side of the communication, operating with a higher level of abstraction than the well-known socket concept, offered by the Quinn\\Rustls library, depending on the transport level adopted. 
    \item \textbf{Send}, pushes serialized data into the socket requiring the transmission to the other side.
    \item \textbf{Recv}, extracts, when available, serialized data from the socket.
\end{itemize}
Note that the network structure works at a lower level with respect to the client structure. The latter relies on an already established connection, according to the transport layer view, to send and receive \acrshort{mqtt} compliant messages, while the former is in charge of opening, maintaining and exchanging data on such connection. Once defined the trait the next step is to define an enumeration containing the different implementations of the network structure. An enumerate is a powerful means that Rust provides to the programmers to define a structure that can contain many variants. In the case of network structure, the implementation leveraged the use of enumeration to discriminate among the different transport layers, dynamically selecting the right branch of code according to the configuration of the network. Each variant, corresponding to one of the available transport layer protocols, relies on a dedicated structure containing the transport layer-specific code, i.e. the socket abstraction associated with such transport protocol offered by the libraries. To clarify the concept the variants available are:
\begin{itemize}
    \item \textbf{TCP}, establishes a plain \acrshort{tcp} connection using a library from the Tokio ecosystem built around standard Rust libraries.
    \item \textbf{TLS}, establishes a plain \acrshort{tcp} connection and upgrades it to a \acrshort{tls} secure session using a library based on Rustls offered by the Tokio ecosystem.
    \item \textbf{\acrshort{quic}}, establish a \acrshort{quic} connection using the Quinn library.
\end{itemize}

\begin{figure}
\centering
\framebox[\columnwidth]{%
\begin{minipage}{0.9\columnwidth}
\dirtree{%
.1 raw-mqtt.
.2 Cargo.toml.
.2 raw-mqtt-lib.
.3 Cargo.toml.
.3 src.
.4 client.
.5 client.rs.
.5 simple\_client.rs.
.5 stream\_client.rs.
.4 client.rs.
.4 lib.rs.
.4 network.
.5 channel.rs.
.5 channel\_network.rs.
.5 network.rs.
.5 server\_verification.rs.
.5 simple\_network.rs.
.5 transport.rs.
.4 network.rs.
.4 utility.
.5 argument\_parser.rs.
.4 utility.rs.
.2 raw-mqtt-cli.
.3 Cargo.toml.
.3 src.
.4 main.rs.
.2 raw-mqtt-stream-cli.
.3 Cargo.toml.
.3 src.
.4 main.rs.
}
\end{minipage}
}
\caption{Code folder structure}
\end{figure}

The code description presented so far hasn't referred to the asynchronous programming paradigm introduced earlier. This is due to the fact that the organization of the crate is independent of the paradigm adopted, although the details of the implementation depend heavily on it. 
\bigbreak
The network sub-crate contains two different implementations of the trait:
\begin{itemize}
    \item \textbf{simple\_network}, standard implementation of the networking operations that operate on the socket offered by the enumeration above described to discriminate between the different transport protocols available.
    \item \textbf{channel\_network}, implementation based on a producer/consumer pattern that allows the decoupling of the application logic defined by the code that will use the library from the networking part defined in this crate.
\end{itemize}

Regarding the first implementation, the behaviour is exactly the one expected by an asynchronous networking operation, i.e. the task that calls the method will suspend in favour of another if the operation can't be immediately completed. The second implementation instead is trickier because the methods don't produce immediately the expected results. The structure once established the connection spawns two separate tasks, one dedicated to writing operations on the socket and one to the reading operations. The interaction with these tasks is possible only via a specialized data structure named channel, a communication mechanism between tasks that can be considered as a queue in which data can be pushed or extracted. In the case of the transmitter task, its execution flow consists of the extraction of data from the queue and the writing of such data to the socket. For the receiver task, the data are received from the socket and then pushed to the queue. The send method results in the insertion of the data to be sent into the queue, while the receive method extracts the data from the second queue, if available.
The experiments to be carried out mainly require send operations, so the receiving part is not so interesting because only acknowledgements will be received. Regarding the transmission the configuration of the queue may have an impact on the metric to evaluate, so a dedicated enumeration containing multiple versions of the queue was defined.
\begin{itemize}
    \item \textbf{Infinite length \acrshort{fifo}}, the queue is managed by a standard \acrshort{fifo} policy, allowing data to be pushed until the system has enough memory to store the queue. 
    \item \textbf{Finite length \acrshort{fifo}}, the queue is managed by a standard \acrshort{fifo} policy, but the number of the available positions is fixed and once the queue is full the task that is trying to push more data blocks until at least a position becomes free.
    \item \textbf{Head-drop}, the queue has only one position, so it should be considered as a buffer rather than a queue, that can be overwritten without blocking the task that pushes data on it.
\end{itemize}

The two network implementations correspond to as many client implementations, both on top of the base client already introduced that define the \acrshort{mqtt} related operations.
\begin{itemize}
    \item simple\_client, it doesn't add any additional features to the base client but acts only as a utility to build the base client plugging the simple\_network structure.
    \item stream\_client, it is based on channel\_network and in addition to the base methods offers the stream\_publish method that allows to decouple the transmission of the message by the associated reception of the acknowledgment. 
\end{itemize}
The former client doesn't require further comment, but the latter deserves a more detailed description because of its greater complexity. In detail once the connection, the one of \acrshort{mqtt} protocol, with the broker is opened a task dedicated to the reception of \acrshort{mqtt} acknowledgements is spawned. This task is in charge of consuming data from the queue employed by the network component, according to what is described for the channel\_network and checking that the received data corresponds to a positive acknowledgement. 

The method stream\_publish takes full advantage of the channel\_network because it limits pushing a message in the queue and leaves the burden of actual transmission and acknowledgement by the dedicated tasks. This approach allows the application logic that calls this method to continue its execution without suspending waiting for a network operation. 

Note that the advantages of one client over the other depend on the application logic, for example in the case of a single execution flow, it isn't worth using the complex stream\_client, but other scenarios may benefit from the decoupling realized by the tasks.

\subsubsubsection{Raw-mqtt-cli}
The first client tool indicated as simple-client, was designed to publish one message with a client configuration dynamically set passing arguments via the command line when the executable is launched. This tool is suitable to evaluate some metrics, mainly energy consumption in this thesis, of a single \acrshort{mqtt} request, composed of three steps:
\begin{enumerate}
    \item The client initializes all the data structures and establishes a connection to the broker, sending a connection message and receiving a positive acknowledgement.
    \item The client builds a message, generating a synthetic payload or copying the input, depending on the arguments, and publishes it according to the configured quality of service, which may require confirmation through acknowledgement.
    \item The client once the publishing has been completed gracefully disconnects from the broker sending a disconnect message and exists. 
\end{enumerate}

The execution flow is quite simple, the asynchronous paradigm is not exploited because only one task is created, the one that executes the three steps, and thus the idle time dictated by the network results in idle time that cannot be used by other execution flows. This behaviour results from the strictly sequential dependency of the three events, i.e. the next cannot start before the previous is fully completed. The client structure from the custom library that is used to build this tool is the "simple\_client". 

\subsubsubsection{Raw-mqtt-stream-cli}
The second client tool indicated as stream-client, was designed to publish multiple messages on the same connection with a fixed generation rate passed as an argument along with the desired duration of the experiment and other parameters. The duration multiplied by the rate results in the total number of messages that will be published by the client that will exit only once all the operations are completed. The scheme of the execution flow mirrors the one of the simple-client above described, however, the second step is transformed into a loop over the total number of messages to be published. The description of the second tool so far seems only an extension of the first tool, which could be considered a particular case for which only one message is published. The big difference that hasn't already been pointed out is that following this approach two major problems arise:
\begin{itemize}
    \item If messages are generated and transmitted by the same execution flows it will result in a coupling of the two operations, but in principle, the generation rate should be as much as possible independent from the transmission rate.
    \item If the quality of service of the published message is greater than level zero, at least an acknowledgement is required, constraining the period between two messages to be greater than \acrshort{rtt} of the network. 
\end{itemize}

These two problems derive from the fact that the single execution flow blocks waiting for network operations, but the idle time may be exploited to generate other data according to the fixed rate. This scenario fits rather well in an asynchronous context because is possible to define multiple concurrent tasks wisely scheduled exploding the idle times and maximizing the usage of the computational resources. The solution to the problem is achieved by adopting the client structure "stream\_mqtt\_client" provided by the custom library. As already described the network operations offered by the methods of the client structure don't immediately involve actual data transmission, but are limited to saving the message to be published on a queue of messages that will eventually managed by a dedicated task that owns the network structure connected to the broker. Moreover, the acknowledgement problem is solved by the introduction of other two tasks, that realize the opposite flow of communication, i.e. a receiver task that owns the network structure receives data from the network and pushes them into a queue that will be emptied by a task dedicated to acknowledgement management. The division into multiple tasks is completely transparent to the tool built around the library client, resulting in a quite easy definition of the main execution flow. 

The only remaining consideration is the synchronization problem between tasks. From an implementation point of view, Rust enforces the adoption of structures that can be safely shared between multiple execution flows, but some bugs in the logic may still cause a stall in the execution due to the cooperative nature of the interaction between tasks. A cooperative interaction means that a task can be scheduled by the asynchronous runtime only if the control is voluntarily yielded by the currently running task that suspends its execution while waiting for an event. In the developed software multiple causes may induce the suspension of a task:
\begin{itemize}
    \item \textbf{Messages producer} 
    \begin{itemize}
        \item Queue is full and the message cannot be pushed into, valid only in the FIFO configuration with finite queue length.
        \item The waiting period has not already elapsed according to the fixed rate.
    \end{itemize}
    \item \textbf{Messages consumer}
    \begin{itemize}
        \item Queue is empty so no message can be extracted from it.
        \item Some networking components are busy and the operation on the socket cannot be immediately completed.
    \end{itemize}
    \item \textbf{Acknowledgment receiver}
    \begin{itemize}
        \item No data is available in the socket, so the task is blocked waiting for new data.
    \end{itemize}
    \item \textbf{Acknowledgment manager}
    \begin{itemize}
        \item Queue is empty so no message can be extracted from it.
    \end{itemize}
\end{itemize}

It's worth recalling once again that the queues between the two couple of tasks are independent, and while the one between messages producer and consumer can be configured by command line the one between the other couple hasn't a fixed length. 

The \ref{fig:raw-mqtt-arch} resumes the complex architecture defined for the raw-mqtt-stream-cli to take full advantage of asynchronous programming.
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/setup/raw_mqtt_arch.pdf}
    \caption{Raw-mqtt software architecture}
    \label{fig:raw-mqtt-arch}
\end{figure}
